An active noise cancellation technique for the CUORE Pulse Tube Cryocoolers

The Cryogenic Underground Observatory for Rare Events (CUORE) experiment at Gran Sasso National Laboratory of INFN searches for neutrinoless double beta decay using TeO2 crystals as cryogenic bolometers. The sensitivity of the measurement heavily depends on the energy resolution of the detector, therefore the success of the experiment stands on the capability to provide an extremely low noise environment. One of the most relevant sources of noise are the mechanical vibrations induced by the five Pulse Tube cryocoolers used on the cryogenic system which houses the detectors. To address this problem, we developed a system to control the relative phases of the pulse tube pressure oscillations, in order to achieve coherent superposition of the mechanical vibrations transmitted to the detectors. In the following, we describe this method and report on the results in applying it to the CUORE system.

==> ref_Books.tex <==
@book{Coleman,
      author         = "Coleman, S.",
      title          = "{Aspects of symmetry}",
      url            = "http://www.cambridge.org/us/academic/subjects/mathematics/%
      						mathematical-physics/aspects-symmetry-selected-erice-lectures",
      year           = "1988",
      publisher		= "Cambridge University Press",
}

@book{El-Mallawany:2002,
      author         = "El-Mallawany, R.~A.~H.",
      title          = "{Tellurite Glasses Handbook: Physical Properties and Data}",
      url            = "https://www.crcpress.com/Tellurite-Glasses-Handbook-Physical-Properties%
      						-and-Data-Second-Edition/ElMallawany/9781439849835",
      publisher      = "CRC Press",
      year           = "2002",
}

@book{EnssSiegfried:2005,
      author         = "Enss, C. and Siegfried, H.",
      title          = "{Low-Temperature Physics}",
      doi            = "10.1007/b137878",
      publisher      = "Springer",
      year           = "2005",
}

@book{Jensen:2000B,
		author 			= "Jensen, C.",
		title 			= "{Controversy and Consensus: Nuclear Beta Decay 1911-1934}",
		year 				= "2000",
      publisher		= "Birkh$\ddot{\text a}$user Basel",
      doi				= "10.1007/978-3-0348-8444-0",
}

@book{KlapdorKleingrothaus:2010zza,
      author         = "Klapdor-Kleingrothaus, H.~V.",
      title          = "{Seventy years of double beta decay: From nuclear physics
                        to beyond-standard-model particle physics}",
      url            = "http://www.worldscibooks.com/physics/6921.html",
      publisher      = "World Scientific",
      year           = "2010",
      SLACcitation   = "%%CITATION = INSPIRE-861595;%%"
}

@book{Krane:1988B,
		author 			= "Krane, K.~S.",
		title 			= "{Introductory nuclear physics}",
		year 				= "1988",
      publisher		= "John Wiley \& Sons",
}

@book{Lesgourgues&al:2013,
      author         = "Lesgourgues, J. and Mangano, G. and Miele, G. and Pastor, S.",
      title          = "{Neutrino Cosmology}",
      url            = "http://www.cambridge.org/it/academic/subjects/physics/%
      						particle-physics-and-nuclear-physics/neutrino-cosmology",
      publisher      = "Cambridge University Press",
      year           = "2013",
}

@book{Pobell:2007,
      author         = "Pobell, F.",
      title          = "{Matter and Methods at Low Temperatures}",
      doi            = "10.1007\%2F978-3-540-46360-3",
      publisher      = "Springer",
      year           = "2007",
}

@book{Rutherford:1930B,
		author 			= "Rutherford, E. and Chadwick, J. and Ellis, C.~D.",
		title 			= "{Radiations from radioactive substances}",
		year 				= "2010",
      publisher		= "Cambridge University Press",
      url				= "http://www.cambridge.org/br/academic/subjects/physics/atomic-physics-molecular-physics-and-
      						chemical-physics/radiations-radioactive-substances",
      note				= "[Reproduction of the original edition (1930)]",
}

@book{Shklovskii&Efros:1984,
      author         = "Shklovskii, B.~I. and Efros, A.~L.",
      title          = "{Electronic Properties of Doped Semiconductors}",
      url            = "http://www.springer.com/la/book/9783662024058",
      publisher      = "Springer",
      year           = "1984",
}

@book{Stahl:2005,
      author         = "Stahl, H.~C.",
      title          = "{Cryogenic Particle Detection}",
      url            = "http://www.springer.com/la/book/9783540201137",
      publisher      = "Springer",
      year           = "2005",
}

@book{Tylecote:1992,
		author 			= "Tylecote, R.~F.",
		title 			= "{A History of Metallurgy}",
		year 				= "1992",
      publisher		= "Maney Publishing for the Institute of Materials",
      note				= "[2nd edition]",
}



==> ref_Others.tex <==
@unpublished{CUORE_BkgBdg,
      author         = "Alduino, C. and others",
		collaboration  = "CUORE Collaboration",
		title          = "{The projected background for the CUORE experiment}",
      year           = "2016",
      note				= "Internal note (unpublished)",
}

@article{Alvarez:1949zz,
		author         = "Alvarez, L.~W.",
		title          = "{A Proposed Experimental Test of the Neutrino Theory}",
		doi            = "10.2172/929771",
		year           = "1949",
		journal        = "Lawrence Berkeley National Laboratory (Berkeley, CA, US), Report UCRL-328",
		reportNumber   = "UCRL-328",
		note				= "(unpublished)",
		SLACcitation   = "%%CITATION = UCRL-328;%%"
}

@manual{Angrik:2005ep,
      author         = "Angrik, J. and others",
      title          = "{KATRIN design report 2004}",
      collaboration  = "KATRIN Collaboration",
      year           = "2005",
      url				= "https://publikationen.bibliothek.kit.edu/270060419",
}
      reportNumber   = "FZKA-7090",
      SLACcitation   = "%%CITATION = FZKA-7090 ETC.;%%",

@unpublished{Ardito:2011SA,
      author         = "Ardito, R. and Perotti, F.",
      title          = "{Seismic analysis of support structure for the CUORE experiment cryostat (in Italian)}",
      year           = "2011",
      note				= "{INFN report (unpublished) [updated in 2016]}",
}

@manual{ASME-BPVC,
		author         = "{American Society of Mechanical Engineers (ASME)}",
		title          = "{Boiler \& Pressure Vessel Code}",
		year           = "2010",
		url            = "https://www.asme.org/products/codes-standards/bpvcviii1-2015-bpvc-section-viiirules",
		note				= "{Sec.\ VIII, Div.\ 1}"
}

@unpublished{Datskov:W1,
      author         = "Datskov, V.",
      title          = "{CUORE wiring port heat load tests}",
      year           = "2011",
      note				= "Internal report (unpublished)",
}

@unpublished{Ferri:PT_pres,
      author         = "Ferri, E.",
      title          = "{Pulse Tubes characterization}",
      year           = "2013",
      note				= "{Internal report (unpublished)}",
}

@incollection{Larrabee:1984,
		editor			= "Larrabee, R.~D.",
		booktitle		= "{Neutron Transmutation Doping of Semiconductor Materials}",
		author			= "Haller, E.~E. and Palaio, N.~P. and Rodder, M. and Hansen, W.~L. and Kreysa, E.",
		title				= "NTD Germanium: A Novel Material for Low Temperature Bolometers",
		year				= "1984",
		doi				= "10.1007/978-1-4613-2695-3_2",
		url				= "http://dx.doi.org/10.1007/978-1-4613-2695-3_2",
		isbn				= "978-1-4612-9675-1",
		publisher		= "Springer US",
		pages				= "21-36",
}

@unpublished{Ligi:W1,
      author         = "Ligi, C. and Iannarelli, M.",
      title          = "{CUORE wiring test at $T<4$\,K}",
      year           = "2014",
      note				= "Internal report (unpublished)",
}

@article{Pauli:1930LE,
      author         = "Pauli, W.~E.",
      title          = "{Open letter to the group of radioactive people at the Gauverein meeting in 
      						T$\ddot{\text u}$bingen (in German)}",
      year           = "December, 4 1930",
      note				= "(unpublished)",
}

@article{Pontecorvo:1946RE,
      author         = "Pontecorvo, B.",
      title          = "{Inverse $\beta^-$ process}",
      year           = "1946",
      journal        = "Chalk River Laboratory (Chalk River, CA), Report PD-205",
      note				= "{(unpublished)}",
}

@article{Salam:1968rm,
      author         = "Salam, A.",
      title          = "{Weak and Electromagnetic Interactions}",
      journal        = "8th Nobel Symposium, Lerum, Sweden, May 1968",
      pages          = "367-377",
      year           = "1968",
      SLACcitation   = "%%CITATION = CONFP,C680519,367;%%",
}
      journal        = "Conf.\ Proc.\ C68-05-19",

@article{Zweig:1981pd,
      author         = "Zweig, G.",
      title          = "{An SU(3) model for strong interaction symmetry and its breaking. Version II}",
      year           = "1964",
      journal        = "CERN Report 8419/TH.412",
      reportNumber   = "CERN-TH-401",
      note				= "[Version I is {\em CERN preprint 8182/TH.401}] (unpublished)",
      SLACcitation   = "%%CITATION = CERN-TH-401;%%"
}



==> ref_Papers.tex <==
% ------------- %
% ----- A ----- %
% ------------- %

@article{Aalseth:1999ji,
      author         = "Aalseth, C.~E. and others",
      title          = "{Neutrinoless double-beta decay of \ce{^{76}Ge}: First results from the International Germanium 
      						Experiment (IGEX) with six isotopically enriched detectors}",
      collaboration  = "IGEX Collaboration",
      journal        = "Phys.\ Rev.\ C",
      volume         = "59",
      pages          = "2108-2113",
      doi            = "10.1103/PhysRevC.59.2108",
      year           = "1999",
      SLACcitation   = "%%CITATION = PHRVA,C59,2108;%%",
}

@article{Aalseth:2002dt,
      author         = "Aalseth, C.~E. and others",
      title          = "{Comment on `Evidence for neutrinoless double beta decay'}",
      journal        = "Mod.\ Phys.\ Lett.\ A",
      volume         = "17",
      year           = "2002",
      pages          = "1475-1478",
      doi            = "10.1142/S0217732302007715",
      SLACcitation   = "%%CITATION = HEP-EX/0202018;%%"
}
      eprint         = "hep-ex/0202018",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Aalseth:2002rf,
      author         = "Aalseth, C.~E. and others",
      title          = "{The IGEX \ce{^{76}Ge} neutrinoless double beta decay experiment: Prospects for next 
      						generation experiments}",
      collaboration  = "IGEX Collaboration",
      journal        = "Phys.\ Rev.\ D",
      volume         = "65",
      pages          = "092007",
      doi            = "10.1103/PhysRevD.65.092007",
      year           = "2002",
      SLACcitation   = "%%CITATION = HEP-EX/0202026;%%",
}
      eprint         = "hep-ex/0202026",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Abe:2008aa,
      author         = "Abe, S. and others",
      title          = "{Precision Measurement of Neutrino Oscillation Parameters with KamLAND}",
      collaboration  = "KamLAND Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "100",
      pages          = "221803",
      doi            = "10.1103/PhysRevLett.100.221803",
      year           = "2008",
      SLACcitation   = "%%CITATION = ARXIV:0801.4589;%%",
}
      eprint         = "0801.4589",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Abgrall:2013rze,
      author         = "Abgrall, N. and others",
      title          = "{The MAJORANA DEMONSTRATOR Neutrinoless Double-Beta Decay Experiment}",
      collaboration  = "MAJORANA Collaboration",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2014",
      pages          = "365432",
      doi            = "10.1155/2014/365432",
      year           = "2014",
      reportNumber   = "LA-UR-13-24815",
      SLACcitation   = "%%CITATION = ARXIV:1308.1633;%%",
}
      eprint         = "1308.1633",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Abreu:1996pa,
      author         = "Abreu, P. and others",
      title          = "{Search for neutral heavy leptons produced in Z decays}",
      collaboration  = "DELPHI Collaboration",
      journal        = "Z.\ Phys.",
      volume         = "C\,74",
      pages          = "57-71",
      doi            = "10.1007/s002880050370",
      year           = "1997",
      reportNumber   = "CERN-PPE-96-195",
      SLACcitation   = "%%CITATION = ZEPYA,C74,57;%%",
}

@article{Ackermann:2012xja,
      author         = "Ackermann, K.~H. and others",
      title          = "{The GERDA experiment for the search of $0\nu\beta\beta$ decay in \ce{^{76}Ge}}",
      collaboration  = "GERDA Collaboration",
      journal        = "Eur.\ Phys.\ J.\ C",
      number         = "3",
      volume         = "73",
      pages          = "2330",
      doi            = "10.1140/epjc/s10052-013-2330-0",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1212.4067;%%",
}
      eprint         = "1212.4067",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Acquafredda:2009zz,
      author         = "Acquafredda, R. and others",
      title          = "{The OPERA experiment in the CERN to Gran Sasso neutrino beam}",
      journal        = "J.\ Instrum.",
      volume         = "4",
      year           = "2009",
      pages          = "P04018",
      doi            = "10.1088/1748-0221/4/04/P04018",
      SLACcitation   = "%%CITATION = JINST,4,P04018;%%"
}

@article{Ade:2013zuv,
      author         = "Ade, P.~A.~R. and others",
      title          = "{Planck 2013 results. XVI. Cosmological parameters}",
      collaboration  = "Planck Collaboration",
      journal        = "Astron.\ Astrophys.",
      volume         = "571",
      pages          = "A16",
      doi            = "10.1051/0004-6361/201321591",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1303.5076;%%",
}
      eprint         = "1303.5076",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",

@article{Ade:2015xua,
      author         = "Ade, P.~A.~R. and others",
      title          = "{Planck 2015 results. XIII. Cosmological parameters}",
      collaboration  = "Planck Collaboration",
      journal        = "Astron.\ Astrophys.",
      volume         = "594",
      year           = "2016",
      pages          = "A13",
      doi            = "10.1051/0004-6361/201525830",
}
      eprint         = "1502.01589",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1502.01589;%%"

@article{Agashe:2014kda,
      author         = "Olive, K.~A. and others",
      title          = "{Review of Particle Physics}",
      collaboration  = "Particle Data Group",
      journal        = "Chin.\ Phys.\ C",
      volume         = "38",
      year           = "2014",
      pages          = "090001",
      doi            = "10.1088/1674-1137/38/9/090001",
      SLACcitation   = "%%CITATION = CHPHD,C38,090001;%%"
}

@article{Agostini:2013mzu,
      author         = "Agostini, M. and others",
      title          = "{Results on Neutrinoless Double-$\beta$ Decay of \ce{^{76}Ge} from Phase I of the GERDA Experiment}",
      collaboration  = "GERDA Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      number         = "12",
      volume         = "111",
      pages          = "122503",
      doi            = "10.1103/PhysRevLett.111.122503",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1307.4720;%%",
}
      eprint         = "1307.4720",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Agostini:2017iyd,
      author         = "Agostini, M. and others",
      title          = "{Background free search for neutrinoless double-$\beta$ decay of \ce{^{76}Ge} with GERDA}",
      collaboration  = "GERDA Collaboration",
      year           = "2017",
      journal        = "Nature",
      volume         = "544",
      number         = "7648",
      pages          = "5-132",
      doi				= "10.1038/nature21717",
}
      eprint         = "1703.00570",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = ARXIV:1703.00570;%%"

@article{Aguirre:2014lua,
      author         = "Artusa, D.~R. and others",
      title          = "{Initial performance of the CUORE-0 experiment}",
      collaboration  = "CUORE Collaboration",
      journal        = "Eur.\ Phys.\ J.\ C",
      volume         = "74",
      year           = "2014",
      number         = "8",
      pages          = "2956",
      doi            = "10.1140/epjc/s10052-014-2956-6",
      SLACcitation   = "%%CITATION = ARXIV:1402.0922;%%"
}
      eprint         = "1402.0922",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Albert:2014awa,
      author         = "Albert, J.~B. and others",
      title          = "{Search for Majorana neutrinos with the first two years of EXO-200 data}",
      collaboration  = "EXO Collaboration",
      journal        = "Nature",
      volume         = "510",
      pages          = "229-234",
      doi            = "10.1038/nature13432",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1402.6956;%%",
}
      eprint         = "1402.6956",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Alduino:2016vjd,
      author         = "Alduino, C. and others",
      title          = "{CUORE-0 detector: design, construction and operation}",
      collaboration  = "CUORE Collaboration",
      journal        = "J.\ Instrum.",
      volume         = "11",
      year           = "2016",
      number         = "07",
      pages          = "P07009",
      doi            = "10.1088/1748-0221/11/07/P07009",
}
      eprint         = "1604.05465",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1604.05465;%%"

@article{Alduino:2016vtd,
      author         = "Alduino, C. and others",
      title          = "{Measurement of the Two-Neutrino Double Beta Decay Half-life of \ce{^{130}Te} with the 
      						CUORE-0 Experiment}",
      collaboration  = "CUORE Collaboration",
      journal        = "Eur.\ Phys.\ J.\ C",
      volume         = "77",
      year           = "2017",
      number         = "1",
      pages          = "13",
      doi            = "10.1140/epjc/s10052-016-4498-6",
}
      eprint         = "1609.01666",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = ARXIV:1609.01666;%%"

@article{Alduino:2016zrl,
      author         = "Alduino, C. and others",
      title          = "{Analysis techniques for the evaluation of the neutrinoless double-$\beta$ decay lifetime 
      						in \ce{^{130}Te} with the CUORE-0 detector}",
      collaboration  = "CUORE Collaboration",
      journal        = "Phys.\ Rev.\ C",
      volume         = "93",
      year           = "2016",
      pages          = "045503",
      doi            = "10.1103/PhysRevC.93.045503",
}
      eprint         = "1601.01334",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = ARXIV:1601.01334;%%",

@article{Alduino:2018,
      author         = "Alduino, C. and others",
      title          = "{First Results from CUORE: A Search for Lepton Number
                        Violation via $0\nu\beta\beta$ Decay of $^{130}$Te}",
      collaboration  = "CUORE Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "120",
      year           = "2018",
      pages          = "132501",
      doi            = "10.1103/PhysRevLett.120.132501",
}
      eprint         = "1710.07988",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = ARXIV:1710.07988;%%",

@article{Alekhin:2015byh,
      author         = "Alekhin, S. and others",
      title          = "{A facility to Search for Hidden Particles at the CERN SPS: the SHiP physics case}",
      journal        = "Rep.\ Prog.\ Phys.",
      volume         = "79",
      year           = "2016",
      number         = "12",
      pages          = "124201",
      doi            = "10.1088/0034-4885/79/12/124201",
}
      eprint         = "1504.04855",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-SPSC-2015-017",
      SLACcitation   = "%%CITATION = ARXIV:1504.04855;%%",

@article{Alessandrello:1988dv,
      author         = "Alessandrello, A. and Camin, D.~V. and Fiorini, E. and Giuliani, A. and Pessina, G.",
      title          = "{Thermal detection of particles using bolometric devices}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "264",
      pages          = "93-97",
      doi            = "10.1016/0168-9002(88)91108-4",
      year           = "1988",
      SLACcitation   = "%%CITATION = NUIMA,A264,93;%%",
}

@article{Alessandrello:1990wd,
      author         = "Alessandrello, A. and Brofferio, C. and Camin, D. and Cremonesi, O. and Fiorini, E. 
      						and Giuliani, A. and Pessina, G.",
      title          = "{A Cryogenic tellurium detector for rare events and gamma-rays}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "247",
      pages          = "442-447",
      doi            = "10.1016/0370-2693(90)90923-T",
      year           = "1990",
      SLACcitation   = "%%CITATION = PHLTA,B247,442;%%",
}

@article{Alessandrello:1991RL,
      author         = "Alessandrello, A. and others",
      title          = "{Measurements on radioactivity of ancient roman lead to be used as
      						shield in searches for rare events}",
      journal        = "Nucl.\ Instrum.\ Meth.\ B",
      volume         = "61",
      pages          = "106-117",
      doi            = "10.1016/0168-583X(91)95569-Y",
      year           = "1991",
}

@article{Alessandrello:1992aa,
      author         = "Alessandrello, A. and others",
      title          = "{Large mass, low temperature, low background detectors}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "315",
      pages          = "263-266",
      doi            = "10.1016/0168-9002(92)90713-E",
      year           = "1992",
}

@article{Alessandrello:1992vk,
      author         = "Alessandrello, A. and others",
      title          = "{A Search for neutrinoless double beta decay of \ce{^{130}Te} with a thermal detector}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "285",
      pages          = "176-182",
      doi            = "10.1016/0370-2693(92)91319-5",
      year           = "1992",
      SLACcitation   = "%%CITATION = PHLTA,B285,176;%%",
}

@article{Alessandrello:1992zc,
      author         = "Alessandrello, A. and others",
      title          = "{Large mass bolometric detectors for double beta decay experiments}",
      journal        = "IEEE Trans.\ Nucl.\ Sci.",
      volume         = "39",
      pages          = "610-614",
      doi            = "10.1109/23.159674",
      year           = "1992",
      SLACcitation   = "%%CITATION = IETNA,39,610;%%",
}

@article{Alessandrello:1993cs,
      author         = "Alessandrello, A. and others",
      title          = "{Milano experiment on $0-\nu$ $\beta \beta$ decay of \ce{^{130}Te} with a thermal detector}",
      journal        = "Nucl.\ Phys.\ B (Proc.\ Suppl.)",
      volume         = "31",
      pages          = "83-87",
      doi            = "10.1016/0920-5632(93)90118-P",
      year           = "1993",
      SLACcitation   = "%%CITATION = NUPHZ,31,83;%%",
}

@article{Alessandrello:1993RL,
      author         = "Alessandrello, A. and others",
      title          = "{Measurements of low radioactive contaminations using bolometric detectors}",
      journal        = "Nucl.\ Instrum.\ Meth.\ B",
      volume         = "83",
      pages          = "539-544",
      doi            = "10.1016/0168-583X(93)95884-8",
      year           = "1991",
}

@article{Alessandrello:1994tm,
      author         = "Alessandrello, A. and others",
      title          = "{A New search for neutrinoless beta beta decay with a thermal detector}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "335",
      pages          = "519-525",
      doi            = "10.1016/0370-2693(94)90388-3",
      year           = "1994",
      SLACcitation   = "%%CITATION = PHLTA,B335,519;%%",
}

@article{Alessandrello:1996ng,
      author         = "Alessandrello, A. and others",
      title          = "{Preliminary results on the performance of a \ce{TeO_2} thermal detector in a search for 
      						direct interactions of WIMPs}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "384",
      year           = "1996",
      pages          = "316-322",
      doi            = "10.1016/0370-2693(96)00573-4",
      SLACcitation   = "%%CITATION = PHLTA,B384,316;%%"
}

@article{Alessandrello:1998bf,
      author         = "Alessandrello, A. and others",
      title          = "{Methods for response stabilization in bolometers for rare decays}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "412",
      year           = "1998",
      pages          = "454-464",
      doi            = "10.1016/S0168-9002(98)00458-6",
      SLACcitation   = "%%CITATION = NUIMA,A412,454;%%"
}

@article{Alessandrello:1998ey,
      author         = "Alessandrello, A. and others",
      title          = "{Preliminary results on double beta decay of \ce{^{130}Te} with an array of twenty 
      						cryogenic detectors}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "433",
      pages          = "156-162",
      doi            = "10.1016/S0370-2693(98)00645-5",
      year           = "1998",
      SLACcitation   = "%%CITATION = PHLTA,B433,156;%%",
}

@article{Alessandrello:1998RL,
      author         = "Alessandrello, A. and others",
      title          = "{Measurements of internal radioactive contamination in samples of 
      						Roman lead to be used in experiments on rare events}",
      journal        = "Nucl.\ Instrum.\ Meth.\ B",
      volume         = "142",
      pages          = "163-172",
      doi            = "10.1016/S0168-583X(98)00279-1",
      year           = "1998",
}

@misc{CUORECryostat_Al,
    author = "Alessandria, F. and others",
title = {{The CUORE cryostat: A 10 mK infrastructure for large bolometric arrays}},
    year = {In preparation}
}


@article{Alessandria:2011vj,
      author         = "Alessandria, F. and others",
      title          = "{CUORE crystal validation runs: results on radioactive
                        contamination and extrapolation to CUORE background}",
      journal        = "Astropart.\ Phys.",
      volume         = "35",
      year           = "2012",
      pages          = "839-849",
      doi            = "10.1016/j.astropartphys.2012.02.008",
}
      SLACcitation   = "%%CITATION = ARXIV:1108.4757;%%"
      eprint         = "1108.4757",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Alessandria:2012zp,
      author         = "Alessandria, F. and others",
      title          = "{Validation of techniques to mitigate copper surface contamination in CUORE}",
      journal        = "Astropart.\ Phys.",
      volume         = "45",
      pages          = "13-22",
      doi            = "10.1016/j.astropartphys.2013.02.005",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1210.1107;%%",
}
      eprint         = "1210.1107",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Alessandria:2013ufa,
		author         = "Alessandria, F. and others",
		title          = "{The 4K outer cryostat for the CUORE experiment: Construction and quality control}",
		journal        = "Nucl.\ Instrum.\ Meth.\ A",
		volume         = "727",
		pages          = "65-72",
		doi            = "10.1016/j.nima.2013.06.015",
		year           = "2013",
}
		eprint         = "1306.1351",
		archivePrefix  = "arXiv",
		primaryClass   = "physics.ins-det",
		SLACcitation   = "%%CITATION = ARXIV:1306.1351;%%",

@article{Alfonso:2015wka,
      author         = "Alfonso, K. and others",
      title          = "{Search for Neutrinoless Double-Beta Decay of $^{130}$Te with CUORE-0}",
      collaboration  = "CUORE Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "115",
      year           = "2015",
      number         = "10",
      pages          = "102502",
      doi            = "10.1103/PhysRevLett.115.102502",
      SLACcitation   = "%%CITATION = ARXIV:1504.02454;%%"
}
      eprint         = "1504.02454",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Allen:2003pta,
      author         = "Allen, S.~W. and Schmidt, R.~W. and Bridle, S.~L.",
      title          = "{A Preference for a non-zero neutrino mass from cosmological data}",
      journal        = "Mon.\ Not.\ Roy.\ Astron.\ Soc.",
      volume         = "346",
      pages          = "593",
      doi            = "10.1046/j.1365-2966.2003.07022.x",
      year           = "2003",
      SLACcitation   = "%%CITATION = ASTRO-PH/0306386;%%",
}
      eprint         = "astro-ph/0306386",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",

@article{Alpert:2014lfa,
      author         = "Alpert, B. and others",
      title          = "{HOLMES - The Electron Capture Decay of $^{163}$Ho to Measure the Electron Neutrino Mass with 
      						sub-eV sensitivity}",
      journal        = "Eur.\ Phys.\ J.\ C",
      volume         = "75",
      year           = "2015",
      number         = "3",
      pages          = "112",
      doi            = "10.1140/epjc/s10052-015-3329-5",
      SLACcitation   = "%%CITATION = ARXIV:1412.5060;%%"
}
      eprint         = "1412.5060",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Ambrosio:1995cx,
      author         = "Ambrosio, M. and others",
      title          = "{Vertical muon intensity measured with MACRO at the Gran Sasso Laboratory}",
      collaboration  = "MACRO Collaboration",
      journal        = "Phys.\ Rev.\ D",
      volume         = "52",
      year           = "1995",
      pages          = "3793-3802",
      doi            = "10.1103/PhysRevD.52.3793",
      reportNumber   = "LNGS-95-03",
      SLACcitation   = "%%CITATION = PHRVA,D52,3793;%%"
}

@article{An:2014bik,
      author         = "An, F.~P. and others",
      title          = "{Search for a Light Sterile Neutrino at Daya Bay}",
      collaboration  = "Daya Bay Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "113",
      year           = "2014",
      pages          = "141802",
      doi            = "10.1103/PhysRevLett.113.141802",
      SLACcitation   = "%%CITATION = ARXIV:1407.7259;%%"
}
      eprint         = "1407.7259",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Andreotti:2009zza,
      author         = "Andreotti, E. and others",
      title          = "{The low radioactivity link of the CUORE experiment}",
      journal        = "J.\ Instrum.",
      volume         = "4",
      year           = "2009",
      pages          = "P09003",
      doi            = "10.1088/1748-0221/4/09/P09003",
      SLACcitation   = "%%CITATION = JINST,4,P09003;%%"
}

@article{Andreotti:2010vj,
      author         = "Andreotti, E. and others",
      title          = "{\ce{^{130}Te} Neutrinoless Double-Beta Decay with CUORICINO}",
      journal        = "Astropart.\ Phys.",
      volume         = "34",
      pages          = "822-831",
      doi            = "10.1016/j.astropartphys.2011.02.002",
      year           = "2011",
      SLACcitation   = "%%CITATION = ARXIV:1012.3266;%%",
}
      eprint         = "1012.3266",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Andreotti:2012zz,
      author         = "Andreotti, E. and Brofferio, C. and Foggetta, L. and Giuliani, A. and Margesin, B. and 
      						Nones, C. and Pedretti, M. and Rusconi, C. and Salvioni, C. and Tenconi, M.",
      title          = "{Production, characterization, and selection of the heating elements for the response 
      						stabilization of the CUORE bolometers}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "664",
      year           = "2012",
      pages          = "161-170",
      doi            = "10.1016/j.nima.2011.10.065",
      SLACcitation   = "%%CITATION = NUIMA,A664,161;%%"
}

@article{Andrews:1949,
      author         = "Andrews, D.~H. and Fowler, R.~D. and Williams, M.~C.",
      title          = "{The Effect of Alpha-particles on a Superconductor}",
      journal        = "Phys.\ Rev.",
      volume         = "76",
      pages          = "154",
      doi            = "10.1103/PhysRev.76.154.2",
      year           = "1949",
}

@article{Andringa:2015tza,
      author         = "Andringa, S. and others",
      title          = "{Current Status and Future Prospects of the SNO+ Experiment}",
      collaboration  = "SNO+ Collaboration",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2016",
      year           = "2015",
      pages          = "6194250",
      doi            = "10.1155/2016/6194250",
      SLACcitation   = "%%CITATION = ARXIV:1508.05759;%%"
}
      eprint         = "1508.05759",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Arblaster:2012Pb,
      author         = "Arblaster, J.~W.",
      title          = "{Thermodynamic properties of lead}",
      journal        = "Comput.\ Coupling Phase Diagrams Thermochem.",
      volume         = "39",
      year           = "2012",
      pages          = "47-53",
      doi				= "10.1016/j.calphad.2012.08.004",
}

@article{Arblaster:2015Cu,
      author         = "Arblaster, J.~W.",
      title          = "{Thermodynamic Properties of Copper}",
      journal        = "J.\ Phase Equil.\ Diff.",
      volume         = "36",
      year           = "2015",
      pages          = "422-444",
      doi				= "10.1007/s11669-015-0399-x",
}

@article{Armenteros:1952NA,
      author         = "Armenteros, R. and Barker, K.~H. and Butler, C.~C. and Cachon, A. and York, C.~M.",
      title          = "{The properties of charged V-particles}",
      journal        = "Phil.\ Mag.",
      volume         = "43",
      year           = "1952",
      pages          = "597-611",
      doi				= "10.1080/14786440608520216",
}
      series			= "7",
      number			= "341",
%Xi baryon observation

@article{Arnaboldi:2002te,
      author         = "Arnaboldi, C. and others",
      title          = "{A Calorimetric search on double beta decay of \ce{^{130}Te}}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "557",
      pages          = "167-175",
      doi            = "10.1016/S0370-2693(03)00212-0",
      year           = "2003",
      SLACcitation   = "%%CITATION = HEP-EX/0211071;%%",
}
      eprint         = "hep-ex/0211071",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Arnaboldi:2005yf,
      author         = "Arnaboldi, C. and Brofferio, C. and Bucci, C. and Gorla, P. and Pessina, G. and Pirro, S.",
      title          = "{1.3\,kg bolometers to search for rare events}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "554",
      year           = "2005",
      pages          = "300-305",
      doi            = "10.1016/j.nima.2005.07.060",
      SLACcitation   = "%%CITATION = NUIMA,A554,300;%%"
}

@article{Arnaboldi:2005xu,
      author         = "Arnaboldi, C. and Bucci, C. and Capelli, S. and Gorla, P. and Guardincerri, E. and Nucciotti, A. 
      						and Pessina, G. and Pirro, S. and Sisti, M.",
      title          = "{The temperature stabilization system of CUORICINO: An array of macro bolometers}",
      journal        = "IEEE Trans.\ Nucl.\ Sci.",
      volume         = "52",
      year           = "2005",
      pages          = "1630-1637",
      doi            = "10.1109/TNS.2005.856758",
      SLACcitation   = "%%CITATION = IETNA,52,1630;%%"
}

@article{Arnaboldi:2008ds,
      author         = "Arnaboldi, C. and others",
      title          = "{Results from a search for the $0\nu\beta\beta$-decay of \ce{^{130}Te}}",
      collaboration  = "CUORICINO",
      journal        = "Phys.\ Rev.\ C",
      volume         = "78",
      pages          = "035502",
      doi            = "10.1103/PhysRevC.78.035502",
      year           = "2008",
      SLACcitation   = "%%CITATION = ARXIV:0802.3439;%%",
}
      eprint         = "0802.3439",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Arnaboldi:2010fj,
      author         = "Arnaboldi, C. and others",
      title          = "{Production of high purity \ce{TeO_2} single crystals for the 
                        study of neutrinoless double beta decay}",
      journal        = "J.\ Cryst.\ Growth",
      number         = "20",
      volume         = "312",
      pages          = "2999-3008",
      doi            = "10.1016/j.jcrysgro.2010.06.034",
      year           = "2010",
      SLACcitation   = "%%CITATION = ARXIV:1005.3686;%%",
}
      eprint         = "1005.3686",
      archivePrefix  = "arXiv",
      primaryClass   = "cond-mat.mtrl-sci",

@article{Arnaboldi:2017aek,
      author         = "Arnaboldi, C. and Carniti, P. and Cassina, L. and Gotti,
                        C. and Liu, X. and Pessina, G.",
      title          = "{The front-end electronics system for the CUORE
                        experiment}",
       journal        = "JINST",
       issue          = "02",
       pages          = "P02026",
       volume         = "13",
      year           = "2018",
      eprint         = "",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1710.06365;%%",
}

@article{Arnold:2011gq,
      author         = "Arnold, R. and others",
      title          = "{Measurement of the Double Beta Decay Half-life of $^{130}Te$ with the NEMO-3 Detector}",
      collaboration  = "NEMO-3 Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "107",
      pages          = "062504",
      doi            = "10.1103/PhysRevLett.107.062504",
      year           = "2011",
      SLACcitation   = "%%CITATION = ARXIV:1104.3716;%%",
}
      eprint         = "1104.3716",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Arnold:2013dha,
      author         = "Arnold, R. and others",
      title          = "{Search for neutrinoless double-beta decay of \ce{^{100}Mo} with the NEMO-3 detector}",
      collaboration  = "NEMO Collaboration",
      journal        = "Phys.\ Rev.\ D",
      number         = "11",
      volume         = "89",
      pages          = "111101",
      doi            = "10.1103/PhysRevD.89.111101",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1311.5695;%%",
}
      eprint         = "1311.5695",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Arnold:2015wpy,
      author         = "Arnold, R. and others",
      title          = "{Result of the search for neutrinoless double-$\beta$ decay in $^{100}$Mo with the NEMO-3 experiment}",
      collaboration  = "NEMO-3 Collaboration",
      year           = "2015",
      journal        = "Phys.\ Rev.\ D",
      volume         = "92",
      number         = "7",
      pages          = "072011",
      doi            = "10.1103/PhysRevD.92.072011",
      SLACcitation   = "%%CITATION = ARXIV:1506.05825;%%"
}
      eprint         = "1506.05825",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Arpesella:1996,
      author         = "Arpesella, C.",
      title          = "{A low background counting facility at laboratori nazionali del Gran Sasso}",
      journal        = "Appl.\ Rad.\ Iso.",
      volume         = "47",
      pages          = "991-996",
      url            = "http://www.sciencedirect.com/science/article/pii/S0969804396000978",
      year           = "1996",
}

@article{Artusa:2014lgv,
      author         = "Artusa, D.~R. and others",
      title          = "{Searching for neutrinoless double-beta decay of \ce{^{130}Te} with CUORE}",
      collaboration  = "CUORE Collaboration",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2015",
      pages          = "879871",
      doi            = "10.1155/2015/879871",
      year           = "2015",
      SLACcitation   = "%%CITATION = ARXIV:1402.6072;%%",
}
      eprint         = "1402.6072",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Artusa:2014wnl,
      author         = "Artusa, D.~R. and others",
      title          = "{Exploring the Neutrinoless Double Beta Decay in the
                        Inverted Neutrino Hierarchy with Bolometric Detectors}",
      collaboration  = "CUORE Collaboration",
      journal        = "Eur.\ Phys.\ J.\ C",
      volume         = "74",
      year           = "2014",
      number         = "10",
      pages          = "3096",
      doi            = "10.1140/epjc/s10052-014-3096-8",
      SLACcitation   = "%%CITATION = ARXIV:1404.4469;%%"
}
      eprint         = "1404.4469",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Aseev:2011dq,
      author         = "Aseev, V.~N. and others",
      title          = "{An upper limit on electron antineutrino mass from Troitsk experiment}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "84",
      pages          = "112003",
      doi            = "10.1103/PhysRevD.84.112003",
      year           = "2011",
      SLACcitation   = "%%CITATION = ARXIV:1108.5034;%%",
}
      eprint         = "1108.5034",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Atre:2009rg,
      author         = "Atre, A. and Han, T. and Pascoli, S. and Zhang, B.",
      title          = "{The Search for Heavy Majorana Neutrinos}",
      journal        = "J.\ High Energy Phys.",
      volume         = "0905",
      pages          = "030",
      doi            = "10.1088/1126-6708/2009/05/030",
      year           = "2009",
      reportNumber   = "FERMILAB-PUB-08-086-T, NSF-KITP-08-54, MADPH-06-1466, DCPT-07-198, IPPP-07-99",
      SLACcitation   = "%%CITATION = ARXIV:0901.3589;%%",
}
      eprint         = "0901.3589",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Auger:2012ar,
      author         = "Auger, M. and others",
      title          = "{Search for Neutrinoless Double-Beta Decay in \ce{^{136}Xe} with EXO-200}",
      collaboration  = "EXO Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "109",
      pages          = "032505",
      doi            = "10.1103/PhysRevLett.109.032505",
      year           = "2012",
      SLACcitation   = "%%CITATION = ARXIV:1205.5608;%%",
}
      eprint         = "1205.5608",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Avignone:2007fu,
      author         = "Avignone, F.~T. and Elliott, S.~R. and Engel, J.",
      title          = "{Double Beta Decay, Majorana Neutrinos, and Neutrino Mass}",
      journal        = "Rev.\ Mod.\ Phys.",
      volume         = "80",
      year           = "2008",
      pages          = "481-516",
      doi            = "10.1103/RevModPhys.80.481",
      reportNumber   = "LA-UR-07-3577",
      SLACcitation   = "%%CITATION = ARXIV:0708.1033;%%"
}
      eprint         = "0708.1033",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Awasthi:2015ota,
      author         = "Awasthi, R.~L. and Dev, P.~S.~B. and Mitra, M.",
      title          = "{Implications of the Diboson Excess for Neutrinoless Double Beta Decay and Lepton Flavor Violation 
      						in TeV Scale Left Right Symmetric Model}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "93",
      year           = "2016",
      number         = "1",
      pages          = "011701",
      doi            = "10.1103/PhysRevD.93.011701",
      reportNumber   = "TUM-HEP-1014-15",
      SLACcitation   = "%%CITATION = ARXIV:1509.05387;%%"
}
      eprint         = "1509.05387",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

% ------------- %
% ----- B ----- %
% ------------- %

@article{Bahcall:2004ip,
      author         = "Bahcall, J.N. and Murayama, H. and Pena-Garay, C.",
      title          = "{What can we learn from neutrinoless double beta decay experiments?}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "70",
      pages          = "033012",
      doi            = "10.1103/PhysRevD.70.033012",
      year           = "2004",
      SLACcitation   = "%%CITATION = HEP-PH/0403167;%%",
}
      eprint         = "hep-ph/0403167",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Bamert:1994qh,
      author         = "Bamert, P. and Burgess, C.P. and Mohapatra, R.N.",
      title          = "{Heavy sterile neutrinos and neutrinoless double beta decay}",
      journal        = "Nucl.\ Phys.\ B",
      volume         = "438",
      pages          = "3-16",
      doi            = "10.1016/0550-3213(94)00575-Y",
      year           = "1995",
      reportNumber   = "MCGILL-94-37, NEIP-94-007, UMD-PP-95-11",
      SLACcitation   = "%%CITATION = HEP-PH/9408367;%%",
}
      eprint         = "hep-ph/9408367",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Barabash:2011aa,
      author         = "Barabash, A.~S.",
      title          = "{SuperNEMO double beta decay experiment}",
      journal        = "J.\ Phys.\ Conf.\ Ser.",
      volume         = "375",
      pages          = "042012",
      doi            = "10.1088/1742-6596/375/1/042012",
      year           = "2012",
      SLACcitation   = "%%CITATION = ARXIV:1112.1784;%%",
}
      eprint         = "1112.1784",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Barabash:2011mf,
      author         = "Barabash, A.~S.",
      title          = "{Double Beta Decay: Historical Review of 75 Years of Research}",
      journal        = "Phys.\ Atom.\ Nucl.",
      volume         = "74",
      year           = "2011",
      pages          = "603-613",
      doi            = "10.1134/S1063778811030070",
      SLACcitation   = "%%CITATION = ARXIV:1104.2714;%%"
}
      eprint         = "1104.2714",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Barea:2009zza,
      author         = "Barea, J. and Iachello, F.",
      title          = "{Neutrinoless double-beta decay in the microscopic interacting boson model}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "79",
      year           = "2009",
      pages          = "044301",
      doi            = "10.1103/PhysRevC.79.044301",
      SLACcitation   = "%%CITATION = PHRVA,C79,044301;%%"
}

@article{Barea:2013bz,
      author         = "Barea, J. and Kotila, J. and Iachello, F.",
      title          = "{Nuclear matrix elements for double-$\beta$ decay}",
      journal        = "Phys.\ Rev.\ C",
      number         = "1",
      volume         = "87",
      pages          = "014315",
      doi            = "10.1103/PhysRevC.87.014315",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1301.4203;%%",
}
      eprint         = "1301.4203",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Barea:2015kwa,
      author         = "Barea, J. and Kotila, J. and Iachello, F.",
      title          = "{$0\nu\beta\beta$ and $2\nu\beta\beta$ nuclear matrix elements in the interacting boson model 
      						with isospin restoration}",
      journal        = "Phys.\ Rev.\ C",
      number         = "3",
      volume         = "91",
      pages          = "034304",
      doi            = "10.1103/PhysRevC.91.034304",
      year           = "2015",
      SLACcitation   = "%%CITATION = PHRVA,C91,034304;%%",
}

@article{Barry:2011wb,
      author         = "Barry, J. and Rodejohann, W. and Zhang, H.",
      title          = "{Light Sterile Neutrinos: Models and Phenomenology}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1107",
      year           = "2011",
      pages          = "091",
      doi            = "10.1007/JHEP07(2011)091",
      SLACcitation   = "%%CITATION = ARXIV:1105.3911;%%"
}
      eprint         = "1105.3911",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Barshay:1974fh,
      author         = "Barshay, S. and Brown, G.E. and Rho, M.",
      title          = "{A New Interpretation of the Pion-Nucleus Optical Potential for Pionic Atoms}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "32",
      year           = "1974",
      pages          = "787",
      doi            = "10.1103/PhysRevLett.32.787",
      note           = "[Erratum: \href{http://journals.aps.org/prl/abstract/10.1103/PhysRevLett.32.1149.3}
      						{Phys.\ Rev.\ Lett.\ {\bf 32}, 1149 (1974)}]",
      reportNumber   = "ITP-SB-73-58",
      SLACcitation   = "%%CITATION = PRLTA,32,787;%%"
}

@article{Baruccietal:2001,
		author			= {Barucci, M. and Brofferio, C. and Giuliani, A. and Gottardi, E. and Peroni, I. and Ventura, G.},
		title				= "{Measurement of Low Temperature Specific Heat of Crystalline \ce{TeO_2} 
								for the Optimization of Bolometric Detectors}",
		journal			= {J.\ Low Temp.\ Phys.},
		number			= {5-6},
		volume			= {123},
		pages				= {303-314},
		doi				= {10.1023/A:1017555615150},
		year				= {2001},
}
		issn				= {0022-2291},
		url				= {http://dx.doi.org/10.1023/A\%3A1017555615150},
		publisher		= {Kluwer Academic Publishers-Plenum Publishers},

@article{Baruccietal:2008SS,
		author			= {Barucci, M. and Lolli, L. and Risegari, L. and Ventura, G.},
		title				= "{Measurement of thermal conductivity of the supports of CUORE cryostat}",
		journal			= {Cryogenics},
		volume			= {48},
		pages				= {166-168},
		doi				= {10.1016/j.cryogenics.2008.03.018},
		year				= {2008},
}

@article{Battye:2013xqa,
      author         = "Battye, R.~A. and Moss, A.",
      title          = "{Evidence for Massive Neutrinos from Cosmic Microwave Background and Lensing Observations}",
      journal        = "Phys.\ Rev.\ Lett.",
      number         = "5",
      volume         = "112",
      pages          = "051303",
      doi            = "10.1103/PhysRevLett.112.051303",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1308.5870;%%",
}
      eprint         = "1308.5870",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",

@article{Beck:1933NA,
      author         = "Beck, G. and Sitte, K.",
      title          = "{On the theory of $\beta$-decay (in German)}",
      journal        = "Z.\ Phys.",
      volume         = "85",
      year           = "1933",
      pages          = "105-119",
      url				= "http://link.springer.com/article/10.1007/BF01340187",
}

@article{Beck:1933NA2,
      author         = "Beck, G.",
      title          = "{Conservation Laws and $\beta$-Emission}",
      journal        = "Nature",
      volume         = "132",
      year           = "1933",
      pages          = "967",
      url				= "http://www.nature.com/nature/journal/v132/n3347/abs/132967a0.html",
}

@article{Becquerel:1896zz,
      author         = "Becquerel, H.",
      title          = "{On the rays emitted by phosphorescence (in French)}",
      journal        = "C.\ R.\ Acad.\ Sci.",
      volume         = "122",
      year           = "1896",
      pages          = "420-421",
      url				= "http://gallica.bnf.fr/ark:/12148/bpt6k30780/f422",
      SLACcitation   = "%%CITATION = INSPIRE-47893;%%"
}

@article{Becquerel:1900NA,
      author         = "Becquerel, H.",
      title          = "{On the dispersion of the radiation from radium in a magnetic field (in French)}",
      journal        = "C.\ R.\ Acad.\ Sci.",
      volume         = "130",
      year           = "1900",
      pages          = "372-376",
      url				= "http://gallica.bnf.fr/ark:/12148/bpt6k3086n/f372",
}

@article{Belli:1989wz,
      author         = "Belli, P. and Bernabei, R. and D'Angelo, S. and De Pascale, M.~P. and Paoluzi, L. and 
      						Santonico, R. and Taborgna, N. and Iucci, N. and Villoresi, G.",
      title          = "{Deep Underground Neutron Flux Measurement With Large Bf$_3$ Counters}",
      journal        = "Nuovo Cim.\ A",
      volume         = "101",
      year           = "1989",
      pages          = "959-966",
      doi            = "10.1007/BF02800162",
      SLACcitation   = "%%CITATION = NUCIA,A101,959;%%"
}

@article{Benes:2005hn,
      author         = "Benes, P. and Faessler, A. and \u{S}imkovic, F. and Kovalenko, S.",
      title          = "{Sterile neutrinos in neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "71",
      pages          = "077901",
      doi            = "10.1103/PhysRevD.71.077901",
      year           = "2005",
      SLACcitation   = "%%CITATION = HEP-PH/0501295;%%",
}
      eprint         = "hep-ph/0501295",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Bergsma:1985is,
      author         = "Bergsma, F. and others",
      title          = "{A Search for Decays of Heavy Neutrinos in the Mass Range (0.5--2.8)\,GeV}",
      collaboration  = "CHARM Collaboration",
      journal        = "Phys.\ Lett.",
      volume         = "B\,166",
      pages          = "473",
      doi            = "10.1016/0370-2693(86)91601-1",
      year           = "1986",
      reportNumber   = "CERN-EP-85-190",
      SLACcitation   = "%%CITATION = PHLTA,B166,473;%%",
}

@article{Bergstrom:2012nx,
      author         = "Bergstrom, J.",
      title          = "{Combining and comparing neutrinoless double beta decay experiments using different nuclei}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1302",
      pages          = "093",
      doi            = "10.1007/JHEP02(2013)093",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1212.4484;%%",
}
      eprint         = "1212.4484",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Bernardi:1987ek,
      author         = "Bernardi, G. and others",
      title          = "{Further Limits on Heavy Neutrino Couplings}",
      journal        = "Phys.\ Lett.",
      volume         = "B\,203",
      pages          = "332",
      doi            = "10.1016/0370-2693(88)90563-1",
      year           = "1988",
      reportNumber   = "CERN-EP/87-234",
      SLACcitation   = "%%CITATION = PHLTA,B203,332;%%",
}

@misc{CUORESuspension,
    author = {Bersani, A. and others},
    title = {{The detector suspension system of the CUORE experiment}},
    year = {In preparation}
}

@article{Best:2015yma,
      author         = "Best, A. and G$\ddot{\text{o}}$rres, J. and Junker, M. and Kratz, K.~L. and Laubenstein, M. and 
      						Long, A. and Nisi, S. and Smith, K. and Wiescher, M.",
      title          = "{Low energy neutron background in deep underground laboratories}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "812",
      year           = "2016",
      pages          = "1-6",
      doi            = "10.1016/j.nima.2015.12.034",
}
      eprint         = "1509.00770",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1509.00770;%%"

@article{Bethe:1934qn,
      author         = "Bethe, H. and Peierls, R.",
      title          = "{The ``neutrino''}",
      journal        = "Nature",
      volume         = "133",
      year           = "1934",
      pages          = "532",
      doi            = "10.1038/133532a0",
      SLACcitation   = "%%CITATION = NATUA,133,532;%%"
}

@article{Beyer:2007MFFT,
      author         = "Beyer, J. and Drung, D. and Kirste, A.",
      title          = "{A Magnetic-Field-Fluctuation Thermometer for the mK Range Based on SQUID-Magnetometry}",
      journal        = "IEEE Trans.\ Appl.\ Supercond.",
      volume         = "17",
      year           = "2007",
      pages          = "760-763",
      doi            = "10.1109/TASC.2007.898265",
}

@article{Bezrukov:2005mx,
      author         = "Bezrukov, F.~L.",
      title          = "{Neutrino minimal standard model predictions for neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "72",
      pages          = "071303",
      doi            = "10.1103/PhysRevD.72.071303",
      year           = "2005",
      SLACcitation   = "%%CITATION = HEP-PH/0505247;%%",
}
      eprint         = "hep-ph/0505247",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Bigagli:2002rl,
      author         = "Bigagli, C.",
      title          = "{The Hispanic lead trade along the attested routes in the western Mediterranean 
      						basin (in Italian)}",
      journal        = "Emp\'uries",
      volume         = "53",
      pages          = "155-194",
      url            = "http://www.raco.cat/index.php/Empuries/issue/view/8023/showToc",
      year           = "2002",
}

@article{Bilenky:1980cx,
      author         = "Bilenky, Samoil M. and Hosek, J. and Petcov, S.~T.",
      title          = "{On Oscillations of Neutrinos with Dirac and Majorana Masses}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "94",
      pages          = "495",
      doi            = "10.1016/0370-2693(80)90927-2",
      year           = "1980",
      reportNumber   = "JINR-E2-80-373",
      SLACcitation   = "%%CITATION = PHLTA,B94,495;%%",
}

@article{Bilenky:2001rz,
      author         = "Bilenky, Samoil M. and Pascoli, S. and Petcov, S.T.",
      title          = "{Majorana neutrinos, neutrino mass spectrum, CP violation and neutrinoless double beta decay. 
      						1. The Three neutrino mixing case}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "64",
      pages          = "053010",
      doi            = "10.1103/PhysRevD.64.053010",
      year           = "2001",
      reportNumber   = "SISSA-1-2001-EP, JANUARY-2001",
      SLACcitation   = "%%CITATION = HEP-PH/0102265;%%",
}
      eprint         = "hep-ph/0102265",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Bilenky:2001xq,
      author         = "Bilenky, Samoil M. and Pascoli, S. and Petcov, S.T.",
      title          = "{Majorana neutrinos, neutrino mass spectrum, CP violation and neutrinoless double beta decay. 
      						2. Mixing of four neutrinos}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "64",
      pages          = "113003",
      doi            = "10.1103/PhysRevD.64.113003",
      year           = "2001",
      eprint         = "hep-ph/0104218",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SISSA-13-2001-EP, TUM-HEP-410-01",
      SLACcitation   = "%%CITATION = HEP-PH/0104218;%%",
}

@article{Bilenky:2012qb,
      author         = "Bilenky, S.~M.",
      title          = "{Neutrino. History of a unique particle}",
      journal        = "Eur.\ Phys.\ J.\ H",
      volume         = "38",
      year           = "2013",
      pages          = "345-404",
      doi            = "10.1140/epjh/e2012-20068-9",
      SLACcitation   = "%%CITATION = ARXIV:1210.3065;%%"
}
      eprint         = "1210.3065",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Bilenky:2014uka,
      author         = "Bilenky, S.~M. and Giunti, C.",
      title          = "{Neutrinoless Double-Beta Decay: a Probe of Physics Beyond the Standard Model}",
      journal        = "Int.\ J.\ Mod.\ Phys.\ A",
      volume         = "30",
      year           = "2015",
      number         = "04n05",
      pages          = "1530001",
      doi            = "10.1142/S0217751X1530001X",
      SLACcitation   = "%%CITATION = ARXIV:1411.4791;%%"
}
      eprint         = "1411.4791",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Biller:2013wua,
      author         = "Biller, S.~D.",
      title          = "{Probing Majorana neutrinos in the regime of the normal mass hierarchy}",
      journal        = "Phys.\ Rev. D",
      number         = "7",
      volume         = "87",
      pages          = "071301",
      doi            = "10.1103/PhysRevD.87.071301",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1306.5654;%%",
}
      eprint         = "1306.5654",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Blennow:2010th,
      author         = "Blennow, M. and Fernandez-Martinez, E. and Lopez-Pavon, J. and Men\'endez, J.",
      title          = "{Neutrinoless double beta decay in seesaw models}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1007",
      year           = "2010",
      pages          = "096",
      doi            = "10.1007/JHEP07(2010)096",
      reportNumber   = "MPP-2010-40, IFT-UAM-CSIC-10-26, FTUAM-10-06,
                        EURONU-WP6-10-18",
      SLACcitation   = "%%CITATION = ARXIV:1005.3240;%%"
}
      eprint         = "1005.3240",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Bochkarev:1987wf,
      author         = "Bochkarev, A.I. and Shaposhnikov, M.E.",
      title          = "{Electroweak Production of Baryon Asymmetry and Upper Bounds on the Higgs and Top Masses}",
      journal        = "Mod.\ Phys.\ Lett.\ A",
      volume         = "2",
      pages          = "417",
      doi            = "10.1142/S0217732387000537",
      year           = "1987",
      reportNumber   = "NBI-HE-87-18",
      SLACcitation   = "%%CITATION = MPLAE,A2,417;%%",
}

@article{Bohr:1913NA2,
      author         = "Bohr, N.",
      title          = "{On the constitution of atoms and molecules. Part II. Systems containing only a Single Nucleus}",
      journal        = "Phil.\ Mag.",
      volume         = "26",
      year           = "1913",
      pages          = "476-502",
      doi				= "10.1080/14786441308634993",
}
      series			= "6",
      number			= "153",

@article{Bonnet:2012kh,
      author         = "Bonnet, F. and Hirsch, M. and Ota, T. and Winter, W.",
      title          = "{Systematic decomposition of the neutrinoless double beta decay operator}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1303",
      year           = "2013",
      pages          = "055",
      doi            = "10.1007/JHEP03(2013)055",
      note           = "[Erratum: \href{http://link.springer.com/article/10.1007\%2FJHEP04\%282014\%29090}
      						{J.\ High Energy Phys. {\bf 1404}, 090 (2014)}]",
}
      reportNumber   = "IFIC-12-079, MPP-2012-134, STUPP-12-212",
      SLACcitation   = "%%CITATION = ARXIV:1212.3045;%%"
      eprint         = "1212.3045",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Borexino:2013xxa,
      author         = "Bellini, G. and others",
      title          = "{SOX: Short distance neutrino Oscillations with BoreXino}",
      collaboration  = "Borexino Collaboration",
      journal        = "J.\ High Energy Phys.",
      volume         = "1308",
      year           = "2013",
      pages          = "038",
      doi            = "10.1007/JHEP08(2013)038",
      SLACcitation   = "%%CITATION = ARXIV:1304.7721;%%"
}
      eprint         = "1304.7721",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Britton:1992xv,
      author         = "Britton, D.~I. and others",
      title          = "{Improved search for massive neutrinos in $\pi^+ \rightarrow e^+\,\nu$ decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "46",
      pages          = "885-887",
      doi            = "10.1103/PhysRevD.46.R885",
      year           = "1992",
      reportNumber   = "TRI-PP-92-29",
      SLACcitation   = "%%CITATION = PHRVA,D46,885;%%",
}

@article{Britton:1992pg,
      author         = "Britton, D.I. and others",
      title          = "{Measurement of the $\pi^+ \rightarrow e^+\,\nu$ branching ratio}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "68",
      pages          = "3000-3003",
      doi            = "10.1103/PhysRevLett.68.3000",
      year           = "1992",
      reportNumber   = "TRI-PP-92-15",
      SLACcitation   = "%%CITATION = PRLTA,68,3000;%%",
}

@article{Brugnera:2013xma,
      author         = "Brugnera, R. and Garfagnini, A.",
      title          = "{Status of the $GERDA$ Experiment at the Laboratori Nazionali del Gran Sasso}",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2013",
      pages          = "506186",
      doi            = "10.1155/2013/506186",
      year           = "2013",
      SLACcitation   = "%%CITATION = 00642,2013,506186;%%",
}

@article{Buccella:2004cd,
      author         = "Buccella, F. and Falcone, D.",
      title          = "{Bounds for neutrinoless double beta decay in SO(10) inspired see-saw models}",
      journal        = "Mod.\ Phys.\ Lett.\ A",
      volume         = "19",
      year           = "2004",
      pages          = "2993",
      doi            = "10.1142/S0217732304016317",
      reportNumber   = "DSF-44-2003, CERN-PH-TH-2004-015",
      SLACcitation   = "%%CITATION = HEP-PH/0404159;%%"
}
      eprint         = "hep-ph/0404159",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Buccheri:2014bma,
      author         = "Buccheri, E. and Capodiferro, M. and Morganti, S. and Orio, F. and Pelosi, A. and Pettinacci, V.",
      title          = "{An assembly line for the construction of ultra-radio-pure detectors}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "768",
      pages          = "130-140",
      doi            = "10.1016/j.nima.2014.09.046",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1405.0852;%%",
}
      eprint         = "1405.0852",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Bucci:2009zwa,
      author         = "Bucci, C. and others",
      title          = "{Background study and Monte Carlo simulations for large-mass bolometers}",
      journal        = "Eur.\ Phys.\ J.\ A",
      volume         = "41",
      year           = "2009",
      number         = "2",
      pages          = "155-168",
      doi            = "10.1140/epja/i2009-10805-7",
      SLACcitation   = "%%CITATION = EPHJA,A41,155;%%"
}

% ------------- %
% ----- C ----- %
% ------------- %

@article{Cabibbo:1963yz,
      author         = "Cabibbo, N.",
      title          = "{Unitary Symmetry and Leptonic Decays}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "10",
      year           = "1963",
      pages          = "531-533",
      doi            = "10.1103/PhysRevLett.10.531",
      SLACcitation   = "%%CITATION = PRLTA,10,531;%%"
}

@article{Capozzi:2013csa,
      author         = "Capozzi, F. and Fogli, G.~L. and Lisi, E. and Marrone, A. and Montanino, D. and Palazzo, A.",
      title          = "{Status of three-neutrino oscillation parameters, circa 2013}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "89",
      pages          = "093018",
      doi            = "10.1103/PhysRevD.89.093018",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1312.2878;%%",
}
      eprint         = "1312.2878",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Capozzi:2016rtj,
      author         = "Capozzi, F. and Lisi, E. and Marrone, A. and Montanino, D. and Palazzo, A.",
      title          = "{Neutrino masses and mixings: Status of known and unknown $3\nu$ parameters}",
		journal        = "Nucl.\ Phys.\ B",
      volume         = "908",
      year           = "2016",
      pages          = "218-234",
      doi            = "10.1016/j.nuclphysb.2016.02.016",
      SLACcitation   = "%%CITATION = ARXIV:1601.07777;%%"
}
      eprint         = "1601.07777",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Cappuzzello:2015oza,
      author         = "Cappuzzello, F. and Agodi, C. and Bond\`i, M. and Carbone, D. and Cavallaro, M. and Foti, A.",
      title          = "{The role of nuclear reactions in the problem of $0\nu\beta\beta$ decay and the NUMEN 
      					project at INFN-LNS}",
      journal        = "J.\ Phys.\ Conf.\ Ser.",
      volume         = "630",
      year           = "2015",
      number         = "1",
      pages          = "012018",
      doi            = "10.1088/1742-6596/630/1/012018",
      SLACcitation   = "%%CITATION = 00462,630,012018;%%"
}
      booktitle      = "{37th Brazilian Workshop on Nuclear Physics Maresias,
                        São Paulo, Brazil, September 8-12, 2014}",

@article{Cardani:2011vg,
      author         = "Cardani, L. and Gironi, L. and Beeman, J.~W. and Dafinei, I. 
      						and Ge, Z. and Pessina, G. and Pirro, S. and Zhu, Y.",
      title          = "{Performance of a large \ce{TeO_2} crystal as a cryogenic bolometer in searching for 
      						neutrinoless double beta decay}",
      journal        = "J.\ Instrum.",
      volume         = "7",
      year           = "2012",
      pages          = "P01020",
      doi            = "10.1088/1748-0221/7/01/P01020",
}
      eprint         = "1106.0568",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = ARXIV:1106.0568;%%"

@article{Catalano:1986M,
      author         = "Catalano, P.~G. and Cavinato, G. and Salvini, F. and Tozzi, M.",
      title          = "{Structural analysis of the Gran Sasso Laboratories of INFN (in Italian)}",
      journal        = "Mem.\ Soc.\ Geol.\ It.",
      volume         = "35",
      year           = "1986",
      pages          = "647-655",
}

@article{Caurier:2004gf,
      author         = "Caurier, E. and Martinez-Pinedo, G. and Nowacki, F. and Poves, A. and Zuker, A.~P.",
      title          = "{The Shell model as unified view of nuclear structure}",
      journal        = "Rev.\ Mod.\ Phys.",
      volume         = "77",
      year           = "2005",
      pages          = "427-488",
      doi            = "10.1103/RevModPhys.77.427",
      SLACcitation   = "%%CITATION = NUCL-TH/0402046;%%"
}
      eprint         = "nucl-th/0402046",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Choi:2002bb,
      author         = "Choi, K. and Jeong, K.S. and Song, W.Y.",
      title          = "{Operator analysis of neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "66",
      pages          = "093007",
      doi            = "10.1103/PhysRevD.66.093007",
      year           = "2002",
      reportNumber   = "KAIST-TH-02-17",
      SLACcitation   = "%%CITATION = HEP-PH/0207180;%%",
}
      eprint         = "hep-ph/0207180",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Chu2006158,
		author			= {Chu, Y. and Li, Y. and Ge, Z. and Wu, G. and Wang, H.},
		title				= "{Growth of the high quality and large size paratellurite single crystals}",
      journal        = "J.\ Cryst.\ Growth",
		number			= {2},
		volume			= {295},
		pages				= {158-161},
		doi				= {10.1016/j.jcrysgro.2006.08.009},
		year				= {2006},
}
		issn				= {0022-0248},
		url				= {http://www.sciencedirect.com/science/article/pii/S0022024806007561},

@article{Cirelli:2004cz,
      author         = "Cirelli, M. and Marandella, G. and Strumia, A. and Vissani, F.",
      title          = "{Probing oscillations into sterile neutrinos with cosmology, astrophysics and experiments}",
      journal        = "Nucl.\ Phys.\ B",
      volume         = "708",
      year           = "2005",
      pages          = "215-267",
      doi            = "10.1016/j.nuclphysb.2004.11.056",
      reportNumber   = "IFUP-TH-2004-2",
      SLACcitation   = "%%CITATION = HEP-PH/0403158;%%"
}
      eprint         = "hep-ph/0403158",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Cirigliano:2004tc,
      author         = "Cirigliano, V. and Kurylov, A. and Ramsey-Musolf, M.~J. and Vogel, P.",
      title          = "{Neutrinoless double beta decay and lepton flavor violation}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "93",
      pages          = "231802",
      doi            = "10.1103/PhysRevLett.93.231802",
      year           = "2004",
      SLACcitation   = "%%CITATION = HEP-PH/0406199;%%",
}
      eprint         = "hep-ph/0406199",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Clemenza:2016RL,
      author         = "Clemenza, M. and others",
      title          = "{Development of a multi-analytical approach for the characterization of ancient Roman lead ingots}",
      journal        = "J.\ Radioanal.\ Nucl.\ Chem.",
      volume         = "311",
      year           = "2017",
      pages          = "1495-1501",
      doi            = "10.1007/s10967-016-5040-x",
}

@article{Cocco:2007za,
      author         = "Cocco, A.G. and Mangano, G. and Messina, M.",
      title          = "{Probing low energy neutrino backgrounds with neutrino capture on beta decaying nuclei}",
      journal        = "J.\ Cosm.\ Astropart.\ Phys.",
      volume         = "0706",
      pages          = "015",
      doi            = "10.1088/1475-7516/2007/06/015",
      year           = "2007",
      SLACcitation   = "%%CITATION = HEP-PH/0703075;%%",
}
      eprint         = "hep-ph/0703075",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Cowan:1953mw,
      author         = "Cowan, C.~L. and Reines, F. and Harrison, F.~B. and Anderson, E.~C. and Hayes, F.~N.",
      title          = "{Large liquid scintillation detectors}",
      journal        = "Phys.\ Rev.",
      volume         = "90",
      year           = "1953",
      pages          = "493-494",
      doi            = "10.1103/PhysRev.90.493",
      SLACcitation   = "%%CITATION = PHRVA,90,493;%%"
}

@article{Cowan:1992xc,
      author         = "Cowan, C.~L. and Reines, F. and Harrison, F.~B. and Kruse, H.~W. and McGuire, A.~D.",
      title          = "{Detection of the free neutrino: A Confirmation}",
      journal        = "Science",
      volume         = "124",
      year           = "1956",
      pages          = "103-104",
      doi            = "10.1126/science.124.3212.103",
      SLACcitation   = "%%CITATION = SCIEA,124,103;%%"
}

@article{Cremonesi:2013vla,
      author         = "Cremonesi, O. and Pavan, M.",
      title          = "{Challenges in Double Beta Decay}",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2014",
      pages          = "951432",
      doi            = "10.1155/2014/951432",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1310.4692;%%"
}
      eprint         = "1310.4692",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{Corruccini:1959HT,
		author			= {Corruccini, R.~J.},
		title				= "{Gaseous heat conduction at low pressures and temperatures}",
		journal			= {Vacuum},
		volume			= {7-8},
		pages				= {19-29},
		doi				= {10.1016/0042-207X(59)90766-3},
		year				= {1959},
}

@article{Cousins:1998a,
		author			= {Cousins, D.~J. and Fisher, S.~N. and Gu\'{e}nault, A.~M. and Haley, R.~P. and Miller, I.~E. 
							and Pickett, G.~R. and Plenderleith, G.~N. and Skyba, P. and Thibault, P.~Y.~A. and Ward, M.~G.},
		title				= "{An Advanced Dilution Refrigerator Designed for the New Lancaster Microkelvin Facility}",
		journal			= {J.\ Low Temp.\ Phys.},
		volume			= {114},
		pages				= {547-570},
		doi				= {10.1023\%2FA\%3A1021862406629},
		year				= {1999},
}

@article{Cuesta:2015iho,
      author         = "Cuesta, A.~J. and Niro, V. and Verde, L.",
      title          = "{Neutrino mass limits: robust information from the power spectrum of galaxy surveys}",
      journal        = "Phys.\ Dark Univ.",
      volume         = "13",
      year           = "2016",
      pages          = "77-86",
      doi            = "10.1016/j.dark.2016.04.005",
}
      eprint         = "1511.05983",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "FTUAM-15-43, IFT-UAM-CSIC-15-125",
      SLACcitation   = "%%CITATION = ARXIV:1511.05983;%%"

@article{Curie_Laborde:1903,
      author         = "Curie, P. and Laborde, A.",
      title          = "{On the heat spontaneously released by the salts of radium (in French)}",
      journal        = "C.\ R.\ Acad.\ Sci.",
      volume         = "136",
      pages          = "673-675",
      year           = "1903",
}
      title          = "{Sur la chaleur d\'egag\'ee spontan\'ement par les sels de radium}",
      url				= "https://fr.wikisource.org/wiki/\%C5\%92uvres_de_Pierre_Curie/44",

@article{Cushman:2016cnv,
      author         = "Cushman, J.~S. and others",
      title          = "{The detector calibration system for the CUORE cryogenic bolometer array}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "844",
      year           = "2017",
      pages          = "32-44",
      doi            = "10.1016/j.nima.2016.11.020",
}
      eprint         = "1608.01607",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1608.01607;%%"

% ------------- %
% ----- D ----- %
% ------------- %

@article{Danby:1962nd,
      author         = "Danby, G. and Gaillard, J.~M. and Goulianos, K.~A. and Lederman, L.~M. and Mistry, N.~B. 
      						and Schwartz, M. and Steinberger, J.",
      title          = "{Observation of High-Energy Neutrino Reactions and the Existence of Two Kinds of Neutrinos}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "9",
      year           = "1962",
      pages          = "36-44",
      doi            = "10.1103/PhysRevLett.9.36",
      SLACcitation   = "%%CITATION = PRLTA,9,36;%%"
}

@article{Davis:1955bi,
      author         = "Davis, Jr., R.",
      title          = "{Attempt to detect the antineutrinos from a nuclear reactor by the 
      						\ce{Cl^{37}}$(\bar{\nu},\el^-)$\ce{Ar^{37}} reaction}",
      journal        = "Phys.\ Rev.",
      volume         = "97",
      year           = "1955",
      pages          = "766-769",
      doi            = "10.1103/PhysRev.97.766",
      SLACcitation   = "%%CITATION = PHRVA,97,766;%%"
}

@article{Dell'Oro:2014yca,
      author         = "Dell'Oro, S. and Marcocci, S. and Vissani, F.",
      title          = "{New expectations and uncertainties on neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "90",
      pages          = "033005",
      doi            = "10.1103/PhysRevD.90.033005",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1404.2616;%%",
}
      eprint         = "1404.2616",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Dell'Oro:2015tia,
      author         = "Dell'Oro, S. and Marcocci, S. and Viel, M. and Vissani, F.",
      title          = "{The contribution of light Majorana neutrinos to neutrinoless double beta decay and cosmology}",
      journal        = "J.\ Cosm.\ Astropart.\ Phys.",
      volume         = "1512",
      year           = "2015",
      pages          = "023",
      doi            = "10.1088/1475-7516/2015/12/023",
      SLACcitation   = "%%CITATION = ARXIV:1505.02722;%%"
}
      eprint         = "1505.02722",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Dell'Oro:2016dbc,
      author         = "Dell'Oro, S. and Marcocci, S.and Viel, M. and Vissani, F.",
      title          = "{Neutrinoless double beta decay: 2015 review}",
      year           = "2016",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2016",
      pages          = "2162659",
      doi            = "10.1155/2016/2162659",
      SLACcitation   = "%%CITATION = ARXIV:1601.07512;%%"
}
      eprint         = "1601.07512",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Deppisch:2012nb,
      author         = "Deppisch, F.~F. and Hirsch, M. and P$\ddot{\text{a}}$s, H.",
      title          = "{Neutrinoless Double Beta Decay and Physics Beyond the Standard Model}",
      journal        = "J.\ Phys.\ G",
      volume         = "39",
      year           = "2012",
      pages          = "124007",
      doi            = "10.1088/0954-3899/39/12/124007",
      reportNumber   = "IFIC-12-56",
      SLACcitation   = "%%CITATION = ARXIV:1208.0727;%%"
}
      eprint         = "1208.0727",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Deppisch:2015yqa,
      author         = "Deppisch, F.~F. and Harz, J. and Hirsch, M. and Huang, W. and P$\ddot{\text{a}}$s, H.",
      title          = "{Falsifying High-Scale Baryogenesis with Neutrinoless Double Beta Decay and Lepton Flavor Violation}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "92",
      year           = "2015",
      number         = "3",
      pages          = "036005",
      doi            = "10.1103/PhysRevD.92.036005",
      reportNumber   = "LCTS-2015-05",
      SLACcitation   = "%%CITATION = ARXIV:1503.04825;%%"
}
      eprint         = "1503.04825",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Dev:2013vxa,
      author         = "Dev, P.~S.~B. and Goswami, S. and Mitra, M. and Rodejohann, W.",
      title          = "{Constraining Neutrino Mass from Neutrinoless Double Beta Decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "88",
      year           = "2013",
      pages          = "091301",
      doi            = "10.1103/PhysRevD.88.091301",
      reportNumber   = "MAN-HEP-2013-08, IPPP-13-26, DCPT-13-52",
      SLACcitation   = "%%CITATION = ARXIV:1305.0056;%%"
}
      eprint         = "1305.0056",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Dev:2015pga,
      author         = "Dev, P.~S.~B. and Mohapatra, R.~N.",
      title          = "{Unified explanation of the $eejj$, diboson and dijet resonances at the LHC}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "115",
      year           = "2015",
      number         = "18",
      pages          = "181803",
      doi            = "10.1103/PhysRevLett.115.181803",
      reportNumber   = "MAN-HEP-2015-14, TUM-HEP-1008-15, UMD-PP-015-012",
      SLACcitation   = "%%CITATION = ARXIV:1508.02277;%%"
}
      eprint         = "1508.02277",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",


@article{Dietrich:2010,
      author         = "Dietrich, M. and Thummes, G.",
      title          = "{Two-stage high frequency pulse tube cooler for refrigeration at 25 K}",
      journal        = "Cryogenics",
      volume         = "50",
      issue          = "4",
      eid 			 = "281-286",
      pages          = "281-286",
      doi            = "https://doi.org/10.1016/j.cryogenics.2010.01.010",
      year           = "2010",
      SLACcitation   = "%%%%",
}

@article{Dirac:1928hu,
      author         = "Dirac, P.~A.~M.",
      title          = "{The Quantum theory of electron}",
      journal        = "Proc.\ Roy.\ Soc.\ Lond.\ A",
      volume         = "117",
      pages          = "610-624",
      doi            = "10.1098/rspa.1928.0023",
      year           = "1928",
      SLACcitation   = "%%CITATION = PRSLA,A117,610;%%",
}

@article{Dirac:1928ej,
      author         = "Dirac, P.~A.~M.",
      title          = "{The Quantum theory of electron. Part II.}",
      journal        = "Proc.\ Roy.\ Soc.\ Lond.\ A",
      volume         = "118",
      pages          = "351",
      doi            = "10.1098/rspa.1928.0056",
      year           = "1928",
      SLACcitation   = "%%CITATION = PRSLA,A118,351;%%",
}

@article{DiValentino:2015sam,
      author         = "Di Valentino, E. and Giusarma, E. and Mena, O. and Melchiorri, A. and Silk, J.",
      title          = "{Cosmological limits on neutrino unknowns versus low redshift priors}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "93",
      year           = "2016",
      number         = "8",
      pages          = "083527",
      doi            = "10.1103/PhysRevD.93.083527",
}
      eprint         = "1511.00975",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1511.00975;%%"

@article{Doi:1980ze,
      author         = "Doi, M. and Kotani, T. and Nishiura, H. and Okuda, K. and Takasugi, E.",
      title          = "{Neutrino Masses and the Double Beta Decay}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "103",
      pages          = "219",
      doi            = "10.1016/0370-2693(81)90746-2",
      year           = "1981",
      reportNumber   = "OS-GE 80-27",
      SLACcitation   = "%%CITATION = PHLTA,B103,219;%%",
}

@article{Doi:1981mj,
      author         = "Doi, M. and Kotani, T. and Nishiura, H. and Okuda, K. and Takasugi, E.",
      title          = "{Neutrino Mass, the Right-handed Interaction and the Double Beta Decay. 
      						2. General Properties and Data Analysis}",
      journal        = "Prog.\ Theor.\ Phys.",
      volume         = "66",
      year           = "1981",
      pages          = "1765",
      doi            = "10.1143/PTP.66.1765",
      note           = "[Erratum: \href{http://ptp.oxfordjournals.org/content/68/1/348}
      						{Prog.\ Theor.\ Phys. {\bf 68}, 348 (1982)}]",
      reportNumber   = "OS-GE-81-29",
      SLACcitation   = "%%CITATION = PTPKA,66,1765;%%"
}

@article{Doi:1982dn,
      author         = "Doi, M. and Kotani, T. and Nishiura, H. and Takasugi, E.",
      title          = "{Double Beta Decay}",
      journal        = "Prog.\ Theor.\ Phys.",
      volume         = "69",
      pages          = "602",
      doi            = "10.1143/PTP.69.602",
      year           = "1983",
      reportNumber   = "OS-GE 82-43",
      SLACcitation   = "%%CITATION = PTPKA,69,602;%%",
}

@article{Doi:1983wv,
      author         = "Doi, M. and Kotani, T. and Nishiura, H. and Takasugi, E.",
      title          = "{The Energy Spectrum and the Angular Correlation in the Beta Beta Decay}",
      journal        = "Prog.\ Theor.\ Phys.",
      volume         = "70",
      pages          = "1353",
      doi            = "10.1143/PTP.70.1353",
      year           = "1983",
      reportNumber   = "OS-GE-83-45, C83-08-04",
      SLACcitation   = "%%CITATION = PTPKA,70,1353;%%",
}

@article{Dolgov:2003sg,
      author         = "Dolgov, A.~D. and Villante, F.~L.",
      title          = "{BBN bounds on active sterile neutrino mixing}",
      journal        = "Nucl.\ Phys.\ B",
      volume         = "679",
      year           = "2004",
      pages          = "261-298",
      doi            = "10.1016/j.nuclphysb.2003.11.031",
      SLACcitation   = "%%CITATION = HEP-PH/0308083;%%"
}
      eprint         = "hep-ph/0308083",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Drukier:1983gj,
      author         = "Drukier, A. and Stodolsky, L.",
      title          = "{Principles and applications of a neutral current detector for neutrino physics and astronomy}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "30",
      pages          = "2295",
      doi            = "10.1103/PhysRevD.30.2295",
      year           = "1984",
      reportNumber   = "MPI-PAE/PTh 36/82",
      SLACcitation   = "%%CITATION = PHRVA,D30,2295;%%",
}

@article{Duerr:2011zd,
      author         = "Duerr, M. and Lindner, M. and Merle, A.",
      title          = "{On the Quantitative Impact of the Schechter-Valle Theorem}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1106",
      pages          = "091",
      doi            = "10.1007/JHEP06(2011)091",
      year           = "2011",
      SLACcitation   = "%%CITATION = ARXIV:1105.0901;%%",
}
      eprint         = "1105.0901",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Dutton:1966a,
      author         = "Dutton, W.~A. Charles Cooper, W.",
      title          = "{The Oxides and Oxyacids of Tellurium}",
      journal        = "Chem.\ Rev.",
      volume         = "66",
      pages          = "657-675",
      doi            = "10.1021/cr60244a003",
      year           = "1966",
}

% ------------- %
% ----- E ----- %
% ------------- %

@article{Efros:1975,
		author  			= "Efros, A.~L. and Shklovskii, B.~I.",
		title   			= "Coulomb gap and low temperature conductivity of disordered systems",
		journal 			= "J.\ Phys.\ C",
		volume  			= "8",
		pages   			= "L49-L51",
		doi     			= "10.1088/0022-3719/8/4/003",
		year    			= "1975",
}

@article{Ekstrom:2014iya,
      author         = "Ekstr$\ddot{\text o}$m, A. and Jansen, G.~R. and Wendt, K.~A. and Hagen, G. and 
      						Papenbrock, T. and Bacca, S. and Carlsson, B. and Gazit, D.",
      title          = "{Effects of three-nucleon forces and two-body currents on Gamow-Teller strengths}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "113",
      year           = "2014",
      number         = "26",
      pages          = "262504",
      doi            = "10.1103/PhysRevLett.113.262504",
      SLACcitation   = "%%CITATION = ARXIV:1406.4696;%%"
}
      eprint         = "1406.4696",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Elliott:1987kp,
      author         = "Elliott, S.~R. and Hahn, A.~A. and Moe, M.~K.",
      title          = "{Direct Evidence for Two Neutrino Double Beta Decay in $^{82}$Se}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "59",
      year           = "1987",
      pages          = "2020-2023",
      doi            = "10.1103/PhysRevLett.59.2020",
      SLACcitation   = "%%CITATION = PRLTA,59,2020;%%"
}

@article{Elliott:2002xe,
      author         = "Elliott, S.~R. and Vogel, P.",
      title          = "{Double beta decay}",
      journal        = "Ann.\ Rev.\ Nucl.\ Part.\ Sci.",
      volume         = "52",
      pages          = "115-151",
      doi            = "10.1146/annurev.nucl.52.050102.090641",
      year           = "2002",
      reportNumber   = "UW-CALT-2002",
      SLACcitation   = "%%CITATION = HEP-PH/0202264;%%",
}
      eprint         = "hep-ph/0202264",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Elliott:2012sp,
      author         = "Elliott, S.~R.",
      title          = "{Recent Progress in Double Beta Decay}",
      journal        = "Mod.\ Phys.\ Lett.\ A",
      volume         = "27",
      year           = "2012",
      pages          = "1230009",
      doi            = "10.1142/S0217732312300091",
      reportNumber   = "LA-UR-12-10209",
      SLACcitation   = "%%CITATION = ARXIV:1203.1070;%%"
}
      eprint         = "1203.1070",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Ellis:1927NA,
      author         = "Ellis, C.~D. and Wooster, W.~A.",
      title          = "{The Average Energy of Disintegration of Radium E}",
      journal        = "Proc.\ R.\ Soc.\ A",
      volume         = "117",
      year           = "1927",
      pages          = "109-123",
      doi				= "10.1098/rspa.1927.0168",
}

@article{Ellis:1927NA2,
      author         = "Ellis, C.~D. and Wooster, W.~A.",
      title          = "{The continuous spectrum of $\beta$-rays}",
      journal        = "Nature",
      volume         = "119",
      year           = "1927",
      pages          = "563-564",
      url				= "http://www.nature.com/nature/journal/v119/n2998/abs/119563c0.html",
}

@article{Ellis:2012ji,
      author         = "Ellis, J. and Janka, H.~T. and Mavromatos, N.~E. and Sakharov, A.~S. and Sarkisyan, E.~K.~G.",
      title          = "{Prospective Constraints on Neutrino Masses from a Core-Collapse Supernova}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "85",
      year           = "2012",
      pages          = "105028",
      doi            = "10.1103/PhysRevD.85.105028",
}
      eprint         = "1202.0248",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KCL-PH-TH-2012-05, LCTS-2012-02, CERN-PH-TH-2012-010",
      SLACcitation   = "%%CITATION = ARXIV:1202.0248;%%"

@article{Engel:2014pha,
      author         = "Engel, J. and \u{S}imkovic, F. and Vogel, P.",
      title          = "{Chiral Two-Body Currents and Neutrinoless Double-Beta Decay in the QRPA}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "89",
      year           = "2014",
      number         = "6",
      pages          = "064308",
      doi            = "10.1103/PhysRevC.89.064308",
      SLACcitation   = "%%CITATION = ARXIV:1403.7860;%%"
}
      eprint         = "1403.7860",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Engel:2016xgb,
      author         = "Engel, J. and Men\'endez, J.",
      title          = "{Status and future of nuclear matrix elements for neutrinoless double-beta decay: a review}",
      journal        = "Rep.\ Prog.\ Phys.",
      volume         = "80",
      year           = "2017",
      number         = "4",
      pages          = "046301",
      doi            = "10.1088/1361-6633/aa5bc5",
}
      eprint         = "1610.06548",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1610.06548;%%"

@article{Erginsoy:1950,
		author			= {Erginsoy, C.},
		title				= "{On the Mechanism of Impurity Band Conduction in Semiconductors}",
		journal			= {Phys.\ Rev.},
		volume			= {80},
		pages				= {1104},
		doi				= {10.1103/PhysRev.80.1104},
		year				= {1950},
}

@article{Ericson:1971,
      author         = "Ericson, M.",
      title          = "{Axial vector nuclear sum rules and exchange effects}",
      journal        = "Ann.\ Phys.",
      volume         = "63",
      year           = "1971",
      pages          = "562-576",
      doi            = "10.1016/0003-4916(71)90029-7",
}

% ------------- %
% ----- F ----- %
% ------------- %

@article{Faessler:2007hu,
      author         = "Faessler, A. and Fogli, G.~L. and Lisi, E. and Rodin, V. and Rotunno, A.~M. and \u{S}imkovic, F.",
      title          = "{Overconstrained estimates of neutrinoless double beta decay within the QRPA}",
      journal        = "J.\ Phys.\ G",
      volume         = "35",
      pages          = "075104",
      doi            = "10.1088/0954-3899/35/7/075104",
      year           = "2008",
      SLACcitation   = "%%CITATION = ARXIV:0711.3996;%%",
}
      eprint         = "0711.3996",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Faessler:2014kka,
      author         = "Faessler, A. and Gonz\'alez, M. and Kovalenko, S. and \u{S}imkovic, F.",
      title          = "{Arbitrary mass Majorana neutrinos in neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "90",
      year           = "2014",
      number         = "9",
      pages          = "096010",
      doi            = "10.1103/PhysRevD.90.096010",
      SLACcitation   = "%%CITATION = ARXIV:1408.6077;%%"
}
      eprint         = "1408.6077",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Fajans:1913NA,
      author         = "Fajans, K.",
      title          = "{The adioactive transformations and the periodic system of the elements (in German)}",
      journal        = "Ber.\ Deut.\ Chem.\ Ges.",
      volume         = "46",
      year           = "1913",
      pages          = "422-439",
      url				= "http://onlinelibrary.wiley.com/doi/10.1002/cber.19130460162/abstract",
}

@article{Fehr200483,
		author 			= "Fehr, M.~A. and Rehkamper, M. and Halliday, A.~N.",
		title 			= "{Application of MC-ICPMS to the precise determination of tellurium isotope compositions 
								in chondrites, iron meteorites and sulfides}",
		journal 			= "Int.\ J.\ Mass Spectrometry ",
		volume 			= "232",
		pages 			= "83-94",
		year 				= "2004",
		doi 				= "http://dx.doi.org/10.1016/j.ijms.2003.11.006",
}
		number 			= "1",
		issn 				= "1387-3806",
		url 				= "http://www.sciencedirect.com/science/article/pii/S1387380603004494",

@article{Feinberg:1958zzb,
      author         = "Feinberg, G.",
      title          = "{Decays of the mu Meson in the Intermediate-Meson Theory}",
      journal        = "Phys.\ Rev.",
      volume         = "110",
      year           = "1958",
      pages          = "1482-1483",
      doi            = "10.1103/PhysRev.110.1482",
      SLACcitation   = "%%CITATION = PHRVA,110,1482;%%"
}

@article{Feinberg:1959zz,
		author 			= {Feinberg, G. and Goldhaber, M.}, 
		title 			= "{Microscopic tests of symmetry principles}",
		volume			= {45}, 
		number 			= {8}, 
		pages 			= {1301-1312}, 
		year 				= {1959}, 
		Url 				= {http://www.pnas.org/content/45/8.toc}, 
		journal 			= "Proc.\ Nat.\ Ac.\ Sci." 
}

@article{Fermi:1933jpa,
      author         = "Fermi, E.",
      title          = "{Trends to a theory of $\beta$ ray emission (in Italian)}",
      journal        = "Ric.\ Sci.",
      volume         = "4",
      year           = "1933",
      pages          = "491-495",
      SLACcitation   = "%%CITATION = RISCA,4,491;%%"
}

@article{Fermi:1934sk,
      author         = "Fermi, E.",
      title          = "{Trends to a theory of $\beta$ radiation (in Italian)}",
      journal        = "Nuovo Cim.",
      volume         = "11",
      pages          = "1-19",
      doi            = "10.1007/BF02959820",
      year           = "1934",
      SLACcitation   = "%%CITATION = NUCIA,11,1;%%",
}

@article{Feruglio:2002af,
      author         = "Feruglio, F. and Strumia, A. and Vissani, F.",
      title          = "{Neutrino oscillations and signals in $\beta$ and $0\nu2\beta$ experiments}",
      journal        = "Nucl.\ Phys.\ B",
      volume         = "637",
      year           = "2002",
      pages          = "345-377",
      doi            = "10.1016/S0550-3213(02)00345-0",
      reportNumber   = "CERN-TH-2002-13, IFUP-TH-2002-1",
      SLACcitation   = "%%CITATION = HEP-PH/0201291;%%"
}
      note           = "[Addendum: Nucl. Phys.B659,359(2003)]",
      eprint         = "hep-ph/0201291",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Feynman:1958ty,
      author         = "Feynman, R.~P. and Gell-Mann, M.",
      title          = "{Theory of Fermi interaction}",
      journal        = "Phys.\ Rev.",
      volume         = "109",
      year           = "1958",
      pages          = "193-198",
      doi            = "10.1103/PhysRev.109.193",
      SLACcitation   = "%%CITATION = PHRVA,109,193;%%"
}

@article{Fiorini:1983yj,
      author         = "Fiorini, E. and Niinikoski, T.~O.",
      title          = "{Low Temperature Calorimetry for Rare Decays}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "224",
      pages          = "83",
      doi            = "10.1016/0167-5087(84)90449-6",
      year           = "1984",
      reportNumber   = "CERN-EP/83-180",
      SLACcitation   = "%%CITATION = NUIMA,A224,83;%%",
}

@article{Fiorini:1998gj,
      author         = "Fiorini, E.",
      title          = "{CUORE: A cryogenic underground observatory for rare events}",
      journal        = "Phys.\ Rep.",
      volume         = "307",
      pages          = "309-317",
      doi            = "10.1016/S0370-1573(98)00060-X",
      year           = "1998",
      SLACcitation   = "%%CITATION = PRPLC,307,309;%%",
}

@article{Fireman:1948,
      author         = "Fireman, E.~L.",
      title          = "{Artificial Radioactive Substances}",
      journal        = "Phys.\ Rev.",
      volume         = "74",
      year           = "1948",
      pages          = "1238",
      doi            = "10.1103/PhysRev.74.1201",
}

@article{Fireman:1949qs,
      author         = "Fireman, E.~L.",
      title          = "{A measurement of the half-life of double beta-decay from \ce{_{50}Sn^{124}}}",
      journal        = "Phys.\ Rev.",
      volume         = "75",
      year           = "1949",
      pages          = "323-324",
      doi            = "10.1103/PhysRev.75.323",
      SLACcitation   = "%%CITATION = PHRVA,75,323;%%"
}

@article{Fireman:1952qt,
      author         = "Fireman, E.~L. and Schwarzer, D.",
      title          = "{A re-investigation of the double beta-decay from \ce{Sn^{124}}}",
      journal        = "Phys.\ Rev.",
      volume         = "86",
      year           = "1952",
      pages          = "451-453",
      doi            = "10.1103/PhysRev.86.451",
      SLACcitation   = "%%CITATION = PHRVA,86,451;%%"
}

@article{Fogli:2004as,
      author         = "Fogli, G.~L. and Lisi, E. and Marrone, A. and Melchiorri,
                        A. and Palazzo, A. and Serra, P. and Silk, J.",
      title          = "{Observables sensitive to absolute neutrino masses:
                        Constraints and correlations from world neutrino data}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "70",
      pages          = "113003",
      doi            = "10.1103/PhysRevD.70.113003",
      year           = "2004",
      SLACcitation   = "%%CITATION = HEP-PH/0408045;%%",
}
      eprint         = "hep-ph/0408045",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Fritzsch:1974nn,
      author         = "Fritzsch, H. and Minkowski, P.",
      title          = "{Unified Interactions of Leptons and Hadrons}",
      journal        = "Annals Phys.",
      volume         = "93",
      pages          = "193-266",
      doi            = "10.1016/0003-4916(75)90211-0",
      year           = "1975",
      reportNumber   = "CALT-68-467",
      SLACcitation   = "%%CITATION = APNYA,93,193;%%",
}

@article{Frossati:1978a,
		author			= {Frossati, G.},
		title				= "{On the Mechanism of Impurity Band Conduction in Semiconductors}",
		journal			= {J.\ Phys.\ Colloques},
		volume			= {39},
		pages				= {C6\textendash 1578},
		doi				= {10.1051/jphyscol:19786604},
		year				= {1978},
}

@article{Froggatt:1978nt,
      author         = "Froggatt, C.~D. and Nielsen, H.~B.",
      title          = "{Hierarchy of Quark Masses, Cabibbo Angles and CP Violation}",
      journal        = "Nucl.\ Phys.\ B",
      volume         = "147",
      year           = "1979",
      pages          = "277",
      doi            = "10.1016/0550-3213(79)90316-X",
      reportNumber   = "CERN-TH-2519",
      SLACcitation   = "%%CITATION = NUPHA,B147,277;%%"
}

@article{Fujita:1965,
      author         = "Fujita, J.~I. and Ikeda, K.",
      title          = "{Existence of isobaric states and beta decay of heavier nuclei}",
      journal        = "Nucl.\ Phys.",
      volume         = "67",
      year           = "1965",
      pages          = "145-177",
      doi            = "10.1016/0029-5582(65)90119-7",
}

@article{Fukugita:1986hr,
      author         = "Fukugita, M. and Yanagida, T.",
      title          = "{Baryogenesis Without Grand Unification}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "174",
      pages          = "45",
      doi            = "10.1016/0370-2693(86)91126-3",
      year           = "1986",
      reportNumber   = "RIFP-641",
      SLACcitation   = "%%CITATION = PHLTA,B174,45;%%",
}

@article{Furry:1939qr,
      author         = "Furry, W.~H.",
      title          = "{On transition probabilities in double beta-disintegration}",
      journal        = "Phys.\ Rev.",
      volume         = "56",
      pages          = "1184-1193",
      doi            = "10.1103/PhysRev.56.1184",
      year           = "1939",
      SLACcitation   = "%%CITATION = PHRVA,56,1184;%%",
}

% ------------- %
% ----- G ----- %
% ------------- %

@article{Gando:2012zm,
      author         = "Gando, A. and others",
      title          = "{Limit on Neutrinoless $\beta\beta$ Decay of \ce{^{136}Xe} from the First Phase of KamLAND-Zen 
      						and Comparison with the Positive Claim in \ce{^{76}Ge}}",
      collaboration  = "KamLAND-Zen Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      number         = "6",
      volume         = "110",
      pages          = "062502",
      doi            = "10.1103/PhysRevLett.110.062502",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1211.3863;%%",
}
      eprint         = "1211.3863",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Gariazzo:2013gua,
      author         = "Gariazzo, S. and Giunti, C. and Laveder, M.",
      title          = "{Light Sterile Neutrinos in Cosmology and Short-Baseline Oscillation Experiments}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1311",
      year           = "2013",
      pages          = "211",
      doi            = "10.1007/JHEP11(2013)211",
      SLACcitation   = "%%CITATION = ARXIV:1309.3192;%%"
}
      eprint         = "1309.3192",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Garwin:1957hc,
      author         = "Garwin, R.~L. and Lederman, L.~M. and Weinrich, M.",
      title          = "{Observations of the Failure of Conservation of Parity and Charge Conjugation in Meson Decays: 
      						The Magnetic Moment of the Free Muon}",
      journal        = "Phys.\ Rev.",
      volume         = "105",
      year           = "1957",
      pages          = "1415-1417",
      doi            = "10.1103/PhysRev.105.1415",
      SLACcitation   = "%%CITATION = PHRVA,105,1415;%%"
}

@article{Gatti:1986cw,
      author         = "Gatti, E. and Manfredi, P.~F.",
      title          = "{Processing the Signals From Solid State Detectors in Elementary Particle Physics}",
      journal        = "Riv.\ Nuovo Cim.",
      volume         = "9",
      year           = "1986",
      pages          = "1-146",
      doi            = "10.1007/BF02822156",
      SLACcitation   = "%%CITATION = RNCIB,9N1,1;%%"
}

@article{GellMann:1955jx,
      author         = "Gell-Mann, M. and Pais, A.",
      title          = "{Behavior of neutral particles under charge conjugation}",
      journal        = "Phys.\ Rev.",
      volume         = "97",
      pages          = "1387-1389",
      doi            = "10.1103/PhysRev.97.1387",
      year           = "1955",
      SLACcitation   = "%%CITATION = PHRVA,97,1387;%%",
}

@article{GellMann:1964nj,
      author         = "Gell-Mann, M.",
      title          = "{A Schematic Model of Baryons and Mesons}",
      journal        = "Phys.\ Lett.",
      volume         = "8",
      year           = "1964",
      pages          = "214-215",
      doi            = "10.1016/S0031-9163(64)92001-3",
      SLACcitation   = "%%CITATION = PHLTA,8,214;%%"
}

@article{GellMann:1980vs,
      author         = "Gell-Mann, M. and Ramond, P. and Slansky, R.",
      title          = "{Complex Spinors and Unified Theories}",
      journal        = "Proceedings of the Supergravity Workshop, Stony Brook, New York, USA, September 1979",
      volume         = "\!\!",
      pages          = "315-321",
      year           = "1979",
      reportNumber   = "PRINT-80-0576",
      SLACcitation   = "%%CITATION = ARXIV:1306.4669;%%",
}
      eprint         = "1306.4669",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      journal        = "Conf.\ Proc.\ C79-09-27",

@article{Georgi:1974sy,
      author         = "Georgi, H. and Glashow, S.~L.",
      title          = "{Unity of All Elementary Particle Forces}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "32",
      pages          = "438-441",
      doi            = "10.1103/PhysRevLett.32.438",
      year           = "1974",
      SLACcitation   = "%%CITATION = PRLTA,32,438;%%",
}

@article{Georgi:1975qb,
      author         = "Georgi, H.",
      title          = "{Unified Gauge Theories}",
      journal        = "Conf.\ Proc.\ C75-01-20",
      volume         = "\!\!",
      year           = "1975",
      SLACcitation   = "%%CITATION = INSPIRE-106900;%%",
}

@article{Ghoshal:2010wt,
      author         = "Ghoshal, P. and Petcov, S.~T.",
      title          = "{Neutrino Mass Hierarchy Determination Using Reactor Antineutrinos}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1103",
      pages          = "058",
      doi            = "10.1007/JHEP03(2011)058",
      year           = "2011",
      reportNumber   = "REF.-ISSI-77-2010-EP",
      SLACcitation   = "%%CITATION = ARXIV:1011.1646;%%",
}
      eprint         = "1011.1646",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Giachero:2013iya,
      author         = "Giachero, A. and Gotti, C. and Maino, M. and Pessina, G.",
      title          = "{Characterization of high impedance connecting links for Bolometric detectors}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "718",
      year           = "2013",
      pages          = "229-230",
      doi            = "10.1016/j.nima.2012.11.140",
      SLACcitation   = "%%CITATION = NUIMA,A718,229;%%"
}
      booktitle      = "{Proc.\ 12th Pisa Meeting on Adv.\ Det., La Biodola, Isola d'Elba, Italy, May 20-26, 2012}",

@article{Gifford:1964a,
		author			= "Gifford, W.~E. and Longsworth, R.~C.",
		title				= "{Pulse-Tube Refrigeration}", 
		journal			= "Trans.\ ASME J.\ Eng.\ Ind.",
		volume			= "3",
		pages				= "264-268",
		doi				= "10.1115/1.3670530",
		year				= "1964",
}

@article{Girardi:2013zra,
      author         = "Girardi, I. and Meroni, A. and Petcov, S.~T.",
      title          = "{Neutrinoless Double Beta Decay in the Presence of Light Sterile Neutrinos}",
      journal        = "J.\ High Energy Phys.",
      volume         = "1311",
      year           = "2013",
      pages          = "146",
      doi            = "10.1007/JHEP11(2013)146",
      reportNumber   = "SISSA-37-2013-FISI",
      SLACcitation   = "%%CITATION = ARXIV:1308.5802;%%"
}
      eprint         = "1308.5802",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Giuliani:2012zu,
      author         = "Giuliani, A. and Poves, A.",
      title          = "{Neutrinoless Double-Beta Decay}",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2012",
      year           = "2012",
      pages          = "857016",
      doi            = "10.1155/2012/857016",
      SLACcitation   = "%%CITATION = 00642,2012,857016;%%"
}

@article{Giusarma:2016phn,
      author         = "Giusarma, E. and Gerbino, M. and Mena, O. and Vagnozzi, S. and Ho, S. and Freese, K.",
      title          = "{Improvement of cosmological neutrino mass bounds}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "94",
      year           = "2016",
      number         = "8",
      pages          = "083522",
      doi            = "10.1103/PhysRevD.94.083522",
}
      eprint         = "1605.04320",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1605.04320;%%"

@article{Glashow:1961tr,
      author         = "Glashow, S.~L.",
      title          = "{Partial Symmetries of Weak Interactions}",
      journal        = "Nucl.\ Phys.",
      volume         = "22",
      pages          = "579-588",
      doi            = "10.1016/0029-5582(61)90469-2",
      year           = "1961",
      SLACcitation   = "%%CITATION = NUPHA,22,579;%%",
}

@article{Glashow:1970gm,
      author         = "Glashow, S.~L. and Iliopoulos, J. and Maiani, L.",
      title          = "{Weak Interactions with Lepton-Hadron Symmetry}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "2",
      year           = "1970",
      pages          = "1285-1292",
      doi            = "10.1103/PhysRevD.2.1285",
      SLACcitation   = "%%CITATION = PHRVA,D2,1285;%%"
}

@article{Glashow:1979nm,
      author         = "Glashow, S.~L.",
      title          = "{The Future of Elementary Particle Physics}",
      journal        = "NATO Sci.\ Ser.\ B",
      volume         = "59",
      pages          = "687",
      year           = "1980",
      reportNumber   = "HUTP-79-A059",
      SLACcitation   = "%%CITATION = HUTP-79-A059 ETC.;%%",
}

@article{GoeppertMayer:1935qp,
      author         = "Goeppert-Mayer, M.",
      title          = "{Double beta-disintegration}",
      journal        = "Phys.\ Rev.",
      volume         = "48",
      pages          = "512-516",
      doi            = "10.1103/PhysRev.48.512",
      year           = "1935",
      SLACcitation   = "%%CITATION = PHRVA,48,512;%%",
}

@article{Goldhaber:1958nb,
      author         = "Goldhaber, M. and Grodzins, L. and Sunyar, A.~W.",
      title          = "{Helicity of Neutrinos}",
      journal        = "Phys.\ Rev.",
      volume         = "109",
      year           = "1958",
      pages          = "1015-1017",
      doi            = "10.1103/PhysRev.109.1015",
      SLACcitation   = "%%CITATION = PHRVA,109,1015;%%"
}

@article{GomezCadenas:2011it,
      author         = "G\'{o}mez-Cadenas, J.~J. and Mart\`in-Albo, J. and Mezzetto, M. and Monrabal, F. and Sorel, M.",
      title          = "{The Search for neutrinoless double beta decay}",
      journal        = "Riv.\ Nuovo Cim.",
      volume         = "35",
      year           = "2012",
      pages          = "29-98",
      doi            = "10.1393/ncr/i2012-10074-9",
      SLACcitation   = "%%CITATION = ARXIV:1109.5515;%%"
}
      eprint         = "1109.5515",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Gomez-Cadenas:2013lta,
      author         = "G\'{o}mez-Cadenas, J.~J. and others",
      title          = "{Present status and future perspectives of the NEXT experiment}",
      collaboration  = "NEXT Collaboration",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2014",
      year           = "2014",
      pages          = "907067",
      doi            = "10.1155/2014/907067",
      reportNumber   = "IFIC-13-46",
      SLACcitation   = "%%CITATION = ARXIV:1307.3914;%%"
}
      eprint         = "1307.3914",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

@article{GonzalezGarcia:2002dz,
      author         = "Gonzalez-Garcia, M.~C. and Nir, Y.",
      title          = "{Neutrino masses and mixing: Evidence and implications}",
      journal        = "Rev.\ Mod.\ Phys.",
      volume         = "75",
      pages          = "345-402",
      doi            = "10.1103/RevModPhys.75.345",
      year           = "2003",
      reportNumber   = "CERN-TH-2002-021, WIS-08-02-FEB-DPP",
      SLACcitation   = "%%CITATION = HEP-PH/0202058;%%",
}
      eprint         = "hep-ph/0202058",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

% ------------- %
% ----- H ----- %
% ------------- %

@article{Halprin:1976mr,
      author         = "Halprin, A. and Minkowski, P. and Primakoff, H. and Rosen, S.~P.",
      title          = "{Double-beta Decay and a Massive Majorana Neutrino}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "13",
      pages          = "2567",
      doi            = "10.1103/PhysRevD.13.2567",
      year           = "1976",
      reportNumber   = "CALT-68-533",
      SLACcitation   = "%%CITATION = PHRVA,D13,2567;%%",
}

@article{Halprin:1983ez,
      author         = "Halprin, A. and Petcov, S.~T. and Rosen, S.~P.",
      title          = "{Effects of Light and Heavy Majorana Neutrinos in Neutrinoless Double Beta Decay}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "125",
      pages          = "335",
      doi            = "10.1016/0370-2693(83)91296-0",
      year           = "1983",
      reportNumber   = "BA-83-15",
      SLACcitation   = "%%CITATION = PHLTA,B125,335;%%",
}

@article{Hamann:2013iba,
      author         = "Hamann, J. and Hasenkamp, J.",
      title          = "{A new life for sterile neutrinos: resolving inconsistencies using hot dark matter}",
      journal        = "J.\ Cosm.\ Astropart.\ Phys.",
      volume         = "1310",
      pages          = "044",
      doi            = "10.1088/1475-7516/2013/10/044",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1308.3255;%%",
}
      eprint         = "1308.3255",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",

@article{Harvey:1990qw,
      author         = "Harvey, J.A. and Turner, M.~S.",
      title          = "{Cosmological baryon and lepton number in the presence of electroweak fermion number violation}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "42",
      pages          = "3344-3349",
      doi            = "10.1103/PhysRevD.42.3344",
      year           = "1990",
      reportNumber   = "FERMILAB-PUB-90-049-A, EFI-90-33",
      SLACcitation   = "%%CITATION = PHRVA,D42,3344;%%",
}

@article{Herrero:1998eq,
      author         = "Herrero, M.",
      title          = "{The Standard model}",
      booktitle      = "{Techniques and Concepts of High-Energy Physics:
                        Proceedings, 10th NATO Advanced Study Institute, St.
                        Croix, USA, June 18-29, 1998}",
      journal        = "NATO Sci. Ser. C",
      volume         = "534",
      year           = "1999",
      pages          = "1-59",
      doi            = "10.1007/978-94-011-4689-0_1",
      eprint         = "hep-ph/9812242",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FTUAM-98-25",
      SLACcitation   = "%%CITATION = HEP-PH/9812242;%%"
}

@article{Heusser:1995wd,
      author         = "Heusser, G.",
      title          = "{Low-radioactivity background techniques}",
      journal        = "Ann.\ Rev.\ Nucl.\ Part.\ Sci.",
      volume         = "45",
      year           = "1995",
      pages          = "543-590",
      doi            = "10.1146/annurev.ns.45.120195.002551",
      SLACcitation   = "%%CITATION = ARNUA,45,543;%%"
}

@article{Hopper:1950NA,
      author         = "Hopper, V.~D. and Biswas, S.",
      title          = "{Evidence Concerning the Existence of the New Unstable Elementary Neutral Particle}",
      journal        = "Phys.\ Rev.",
      volume         = "80",
      year           = "1950",
      pages          = "1099-1100",
      doi            = "10.1103/PhysRev.80.1099",
}
% lambda baryon observation

@article{Houlei:2012,
      author         = "Houlei, C. and Nana, X. and Jingtao, L. and Luwei, Y.",
      title          = "{Vibration reduction of pulse tube cryocooler driven by single piston compressor}",
      journal        = "Cryogenics",
      volume         = "52",
      issue          = "12",
      eid 			 = "816-818",
      pages          = "816-818",
      doi            = "https://doi.org/10.1016/j.cryogenics.2012.09.005",
      year           = "2012",
      SLACcitation   = "%%%%",
}


@article{Hyvarinen:2015bda,
      author         = "Hyvarinen, J. and Suhonen, J.",
      title          = "{Nuclear matrix elements for $0\nu\beta\beta$ decays with light or heavy Majorana-neutrino exchange}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "91",
      year           = "2015",
      number         = "2",
      pages          = "024613",
      doi            = "10.1103/PhysRevC.91.024613",
      SLACcitation   = "%%CITATION = PHRVA,C91,024613;%%"
}

% ------------- %
% ----- I ----- %
% ------------- %

% ------------- %
% ----- J ----- %
% ------------- %

@article{Ikushima:2008,
      author         = "Ikushima, Y. and Li, R. and Tomaru, T. and Sato, N. and Suzuki, T. and Haruyama, T. and Shintomi, T. and Yamamoto, A.",
      title          = "{Ultra-low-vibration pulse-tube cryocooler system – cooling capacity and vibration}",
      journal        = "Cryogenics",
      volume         = "48",
      eid 			 = "9-10, 406-412",
      pages          = "406-412",
      doi            = "https://doi.org/10.1016/j.cryogenics.2008.04.001",
      year           = "2008",
      SLACcitation   = "%%%%",
}


@article{Jackson:1957zzb,
      author         = "Lande, K. and Lederman, L.~M. and Chinowsky, W.",
      title          = "{Report on Long-Lived K0 Mesons}",
      journal        = "Phys.\ Rev.",
      volume         = "105",
      pages          = "1925-1927",
      doi            = "10.1103/PhysRev.105.1925.2",
      year           = "1957",
      SLACcitation   = "%%CITATION = PHRVA,105,1925;%%",
}

@article{Joule:1852Th,
		author			= "Joule, J.~P. and Thomson, W.",
		title				= "{On the thermal effects experienced by air in rushing through small apertures}", 
		journal			= "Phil.\ Mag.",
		volume			= "4",
		pages				= "481-492",
		doi				= "10.1017/CBO9780511995187.019",
		year				= "1852"
}

% ------------- %
% ----- K ----- %
% ------------- %

@article{Kajantie:1995kf,
      author         = "Kajantie, K. and Laine, M. and Rummukainen, K. and Shaposhnikov, M.~E.",
      title          = "{The Electroweak phase transition: A Nonperturbative analysis}",
      journal        = "Nucl.\ Phys.\ B",
      volume         = "466",
      pages          = "189-258",
      doi            = "10.1016/0550-3213(96)00052-1",
      year           = "1996",
      reportNumber   = "CERN-TH-95-263, HD-THEP-95-44, HU-TFT-95-57, IUHET-318",
      SLACcitation   = "%%CITATION = HEP-LAT/9510020;%%",
}
      eprint         = "hep-lat/9510020",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",

@article{KamLAND-Zen:2016pfg,
      author         = "Gando, A. and others",
      title          = "{Search for Majorana Neutrinos near the Inverted Mass Hierarchy Region with KamLAND-Zen}",
      collaboration  = "KamLAND-Zen Collaboration",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "117",
      year           = "2016",
      number         = "8",
      pages          = "082503",
      doi            = "10.1103/PhysRevLett.117.109903",
}
      note           = "[Addendum: Phys. Rev. Lett.117,no.10,109903(2016)]",
      eprint         = "1605.02889",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1605.02889;%%"

@article{Keung:1983uu,
      author         = "Keung, W.~Y. and Senjanovic, G.",
      title          = "{Majorana Neutrinos and the Production of the Right-handed Charged Gauge Boson}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "50",
      pages          = "1427",
      doi            = "10.1103/PhysRevLett.50.1427",
      year           = "1983",
      reportNumber   = "BNL-32872",
      SLACcitation   = "%%CITATION = PRLTA,50,1427;%%",
}

@article{KlapdorKleingrothaus:2000sn,
      author         = "Klapdor-Kleingrothaus, H.~V. and others",
      title          = "{Latest results from the Heidelberg-Moscow double beta decay experiment}",
      journal        = "Eur.\ Phys.\ J.\ A",
      volume         = "12",
      pages          = "147-154",
      doi            = "10.1007/s100500170022",
      year           = "2001",
      SLACcitation   = "%%CITATION = HEP-PH/0103062;%%",
}
      eprint         = "hep-ph/0103062",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{KlapdorKleingrothaus:2001ke,
      author         = "Klapdor-Kleingrothaus, H.~V. and Dietz, A. and Harney, H.~L. and Krivosheina, I.~V.",
      title          = "{Evidence for neutrinoless double beta decay}",
      journal        = "Mod.\ Phys.\ Lett.\ A",
      volume         = "16",
      year           = "2001",
      pages          = "2409-2420",
      doi            = "10.1142/S0217732301005825",
      SLACcitation   = "%%CITATION = HEP-PH/0201231;%%"
}
      eprint         = "hep-ph/0201231",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{KlapdorKleingrothaus:2004wj,
      author         = "Klapdor-Kleingrothaus, H.~V. and Krivosheina, I.~V. and Dietz, A. and Chkvorets, O.",
      title          = "{Search for neutrinoless double beta decay with enriched Ge-76 in Gran Sasso 1990-2003}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "586",
      year           = "2004",
      pages          = "198-212",
      doi            = "10.1016/j.physletb.2004.02.025",
      SLACcitation   = "%%CITATION = HEP-PH/0404088;%%"
}
      eprint         = "hep-ph/0404088",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{KlapdorKleingrothaus:2006ff,
      author         = "Klapdor-Kleingrothaus, H.~V. and Krivosheina, I.~V.",
      title          = "{The evidence for the observation of 0nu beta beta decay:
                        The identification of 0nu beta beta events from the full spectra}",
      journal        = "Mod.\ Phys.\ Lett.\ A",
      volume         = "21",
      year           = "2006",
      pages          = "1547-1566",
      doi            = "10.1142/S0217732306020937",
      SLACcitation   = "%%CITATION = MPLAE,A21,1547;%%"
}

@article{Klein:1929zz,
      author         = "Klein, O.",
      title          = "{The Reflection of electrons at a step potential, following Dirac's relativistic 
      						dynamics (in German)}",
      journal        = "Z.\ Phys.",
      volume         = "53",
      year           = "1929",
      pages          = "157",
      doi            = "10.1007/BF01339716",
      SLACcitation   = "%%CITATION = ZEPYA,53,157;%%"
}

@article{Kodama:2000mp,
      author         = "Kodama, K. and others",
      title          = "{Observation of tau neutrino interactions}",
      collaboration  = "DONUT Collaboration",
      journal        = "Phys.\ Lett.\ B",
      volume         = "504",
      year           = "2001",
      pages          = "218-224",
      doi            = "10.1016/S0370-2693(01)00307-0",
      reportNumber   = "FERMILAB-PUB-00-335-E",
      SLACcitation   = "%%CITATION = HEP-EX/0012035;%%"
}
      eprint         = "hep-ex/0012035",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Kolac&al:1984,
		author			= "Kol\'a\u{c}, M. and Neganov, B.~S. and Sahling, S.",
		title				= "{Low Temperature Heat Release from Copper: Ortho-Para Conversion of Hydrogen}",
		journal			= "J.\ Low Temp.\ Phys.",
		volume			= "59",
		pages				= "547-559",
		doi				= "10.1007/BF00682449",
		year				= "1985"
}
		number			={5-6},
		url				={http://www.scopus.com/inward/
								record.url?eid=2-s2.0-0022077165&partnerID=40&md5=1ee8006577c9e56507c25c0a276f2510},

@article{Kotila:2012zza,
      author         = "Kotila, J. and Iachello, F.",
      title          = "{Phase space factors for double-$\beta$ decay}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "85",
      pages          = "034316",
      doi            = "10.1103/PhysRevC.85.034316",
      year           = "2012",
      SLACcitation   = "%%CITATION = ARXIV:1209.5722;%%",
}
      eprint         = "1209.5722",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Kovalenko:2009td,
      author         = "Kovalenko, S. and Lu, Z. and Schmidt, I.",
      title          = "{Lepton Number Violating Processes Mediated by Majorana Neutrinos at Hadron Colliders}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "80",
      pages          = "073014",
      doi            = "10.1103/PhysRevD.80.073014",
      year           = "2009",
      SLACcitation   = "%%CITATION = ARXIV:0907.2533;%%",
}
      eprint         = "0907.2533",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Kovalenko:2013eba,
      author         = "Kovalenko, S. and Krivoruchenko, M.~I. and \u{S}imkovic, F.",
      title          = "{Neutrino propagation in nuclear medium and neutrinoless double-beta decay}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "112",
      year           = "2014",
      number         = "14",
      pages          = "142503",
      doi            = "10.1103/PhysRevLett.112.142503",
      SLACcitation   = "%%CITATION = ARXIV:1311.4200;%%"
}
      eprint         = "1311.4200",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Kraus:2004zw,
      author         = "Kraus, C. and others",
      title          = "{Final results from phase II of the Mainz neutrino mass search in tritium beta decay}",
      journal        = "Eur.\ Phys.\ J.\ C",
      volume         = "40",
      pages          = "447-468",
      doi            = "10.1140/epjc/s2005-02139-7",
      year           = "2005",
      SLACcitation   = "%%CITATION = HEP-EX/0412056;%%",
}
      eprint         = "hep-ex/0412056",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Kroeger:1977,
      author         = "Kroeger, F.~R. and Swenson, C.~A.",
      title          = "{Absolute linear thermal-expansion measurements on copper and aluminum from 5 to 320 K }",
      journal        = "J.\ Appl.\ Phys.",
      number         = "3",
      volume         = "48",
      pages          = "853-864",
      url            = "http://dx.doi.org/10.1063/1.323746",
      year           = "1977",
}

@article{Kurie:1936KP,
      author         = "Kurie, F.~N.~D. and Richardson, J.~R. and Paxton, C.",
      title          = "{The Radiations Emitted from Artificially Produced Radioactive Substances. 
      						I. The Upper Limits and Shapes of the $\beta$-Ray Spectra from Several Elements}",
      journal        = "Phys.\ Rev.",
      volume         = "49",
      pages          = "368",
      doi            = "10.1103/PhysRev.49.368",
      year           = "1936",
}

@article{Kuzmin:1985mm,
      author         = "Kuzmin, V.~A. and Rubakov, V.~A. and Shaposhnikov, M.~E.",
      title          = "{On the Anomalous Electroweak Baryon Number Nonconservation in the Early Universe}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "155",
      pages          = "36",
      doi            = "10.1016/0370-2693(85)91028-7",
      year           = "1985",
      reportNumber   = "IC/85/8",
      SLACcitation   = "%%CITATION = PHLTA,B155,36;%%",
}

% ------------- %
% ----- L ----- %
% ------------- %

@article{Laing:2016puy,
      author         = "Laing, A.",
      title          = "{The NEXT double beta decay experiment}",
      booktitle      = "{Proceedings, 14th International Conference on Topics in
                        Astroparticle and Underground Physics (TAUP 2015): Torino,
                        Italy, September 7-11, 2015}",
      collaboration  = "NEXT",
      journal        = "J. Phys. Conf. Ser.",
      volume         = "718",
      year           = "2016",
      number         = "6",
      pages          = "062033",
      doi            = "10.1088/1742-6596/718/6/062033",
      SLACcitation   = "%%CITATION = 00462,718,062033;%%"
}
@article{Landau:1957tp,
      author         = "Landau, L.~D.",
      title          = "{On the conservation laws for weak interactions}",
      journal        = "Nucl.\ Phys.",
      volume         = "3",
      pages          = "127-131",
      doi            = "10.1016/0029-5582(57)90061-5",
      year           = "1957",
      SLACcitation   = "%%CITATION = NUPHA,3,127;%%",
}

@article{Lande:1956pf,
      author         = "Lande, K. and Booth, E.~T. and Impeduglia, J. and Lederman, L.~M. and Chinowsky, W.",
      title          = "{Observation of Long-Lived Neutral V Particles}",
      journal        = "Phys.\ Rev.",
      volume         = "103",
      pages          = "1901-1904",
      doi            = "10.1103/PhysRev.103.1901",
      year           = "1956",
      SLACcitation   = "%%CITATION = PHRVA,103,1901;%%",
}

@article{Lee:1956qn,
      author         = "Lee, T.~D. and Yang, C.~N.~F.",
      title          = "{Question of Parity Conservation in Weak Interactions}",
      journal        = "Phys.\ Rev.",
      volume         = "104",
      year           = "1956",
      pages          = "254-258",
      doi            = "10.1103/PhysRev.104.254",
      SLACcitation   = "%%CITATION = PHRVA,104,254;%%"
}

@article{Lee:1957qr,
      author         = "Lee, T.~D. and Yang, C.~N.",
      title          = "{Parity Nonconservation and a Two Component Theory of the Neutrino}",
      journal        = "Phys.\ Rev.",
      volume         = "105",
      pages          = "1671-1675",
      doi            = "10.1103/PhysRev.105.1671",
      year           = "1957",
      SLACcitation   = "%%CITATION = PHRVA,105,1671;%%",
}

@article{Lee:1965hi,
      author         = "Lee, T.~D. and Wolfenstein, L.",
      title          = "{Analysis of CP Noninvariant Interactions and the $K_1^0$, $K_2^0$ System}",
      journal        = "Phys.\ Rev.",
      volume         = "138",
      pages          = "B1490-B1496",
      doi            = "10.1103/PhysRev.138.B1490",
      year           = "1965",
      SLACcitation   = "%%CITATION = PHRVA,138,B1490;%%",
}

@article{Lesgourgues:2014zoa,
      author         = "Lesgourgues, J. and Pastor, S.",
      title          = "{Neutrino cosmology and Planck}",
      journal        = "New J.\ Phys.",
      volume         = "16",
      year           = "2014",
      pages          = "065002",
      doi            = "10.1088/1367-2630/16/6/065002",
      reportNumber   = "MITP-14-015",
      SLACcitation   = "%%CITATION = ARXIV:1404.1740;%%"
}
      eprint         = "1404.1740",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Levinson:1980,
      author         = "Levinson, Y.~B.",
      title          = "{Propagation of Nonequilibrium Phonons with Frequency Down-conversion (Anthracene)}",
      journal        = "Mol.\ Cryst.\ Liq.\ Cryst.",
      volume         = "57",
      year           = "1980",
      pages          = "23-38",
      doi            = "10.1080/00268948008069816",
}

@article{Lisi:2015yma,
      author         = "Lisi, E. and Rotunno, A. and \u{S}imkovic, F.",
      title          = "{Degeneracies of particle and nuclear physics
                        uncertainties in neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "92",
      pages          = "093004",
      doi            = "10.1103/PhysRevD.92.093004",
      year           = "2015",
      SLACcitation   = "%%CITATION = ARXIV:1506.04058;%%"
}
      eprint         = "1506.04058",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{London:1962zz,
      author         = "London, H. and Clarke, G.~R. and Mendoza, E.",
      title          = "{Osmotic Pressure of He$^3$ in Liquid He$^4$, with Proposals
                        for a Refrigerator to Work below 1$^\circ$K}",
      journal        = "Phys.\ Rev.",
      volume         = "128",
      year           = "1962",
      pages          = "1992-2005",
      doi            = "10.1103/PhysRev.128.1992",
      SLACcitation   = "%%CITATION = PHRVA,128,1992;%%"
}

@article{Long:2014zva,
      author         = "Long, A.~J. and Lunardini, C. and Sabancilar, E.",
      title          = "{Detecting non-relativistic cosmic neutrinos by capture
                        on tritium: phenomenology and physics potential}",
      journal        = "J.\ Cosm.\ Astropart.\ Phys.",
      volume         = "1408",
      pages          = "038",
      doi            = "10.1088/1475-7516/2014/08/038",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1405.7654;%%",
}
      eprint         = "1405.7654",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{LopezPavon:2012zg,
      author         = "Lopez-Pavon, J. and Pascoli, S. and Wong, C.",
      title          = "{Can heavy neutrinos dominate neutrinoless double beta decay?}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "87",
      year           = "2013",
      number         = "9",
      pages          = "093007",
      doi            = "10.1103/PhysRevD.87.093007",
      reportNumber   = "IPPP-12-68, DCPT-12-136",
      SLACcitation   = "%%CITATION = ARXIV:1209.5342;%%"
}
      eprint         = "1209.5342",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Loredo:2001rx,
      author         = "Loredo, T.~J. and Lamb, D.~Q.",
      title          = "{Bayesian analysis of neutrinos observed from supernova SN-1987A}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "65",
      pages          = "063002",
      doi            = "10.1103/PhysRevD.65.063002",
      year           = "2002",
      SLACcitation   = "%%CITATION = ASTRO-PH/0107260;%%",
}
      eprint         = "astro-ph/0107260",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",

@article{Luty:1992un,
      author         = "Luty, M. A.",
      title          = "{Baryogenesis via leptogenesis}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "45",
      year           = "1992",
      pages          = "455-465",
      doi            = "10.1103/PhysRevD.45.455",
      SLACcitation   = "%%CITATION = PHRVA,D45,455;%%"
}

% ------------- %
% ----- M ----- %
% ------------- %

@article{Martin-Albo:2015rhw,
      author         = "Mart\`in-Albo, J. and others",
      title          = "{Sensitivity of NEXT-100 to neutrinoless double beta decay}",
      collaboration  = "NEXT Collaboration",
      journal        = "J.\ High Energy Phys.",
      volume         = "05",
      year           = "2016",
      pages          = "159",
      doi            = "10.1007/JHEP05(2016)159",
}
      eprint         = "1511.09246",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1511.09246;%%"

@article{Majorana:1937vz,
      author         = "Majorana, E.",
      title          = "{Theory of the Symmetry of Electrons and Positrons (in Italian)}",
      journal        = "Nuovo Cim.",
      volume         = "14",
      pages          = "171-184",
      doi            = "10.1007/BF02961314",
      year           = "1937",
      reportNumber   = "RX-888",
      SLACcitation   = "%%CITATION = NUCIA,14,171;%%",
}

@article{McCarty:2009He,
      author         = "Mc Carty, R.~D",
      title          = "{Thermodynamic Properties of Helium 4 from 2 to 1500\,K at Pressures to $10^8$\,Pa}",
      journal        = "J.\ Phys.\ Chem.\ Ref.\ Data",
      volume         = "2",
      year           = "2009",
      pages          = "139-151",
      doi            = "10.1063/1.3253133",
}

@article{Menendez:2008jp,
      author         = "Men\'{e}ndez, J. and Poves, A. and Caurier, E. and Nowacki, F.",
      title          = "{Disassembling the Nuclear Matrix Elements of the Neutrinoless beta beta Decay}",
      journal        = "Nucl.\ Phys.\ A",
      volume         = "818",
      year           = "2009",
      pages          = "139-151",
      doi            = "10.1016/j.nuclphysa.2008.12.005",
      SLACcitation   = "%%CITATION = ARXIV:0801.3760;%%"
}
      eprint         = "0801.3760",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Menendez:2011qq,
      author         = "Men\'{e}ndez, J. and Gazit, D. and Schwenk, A.",
      title          = "{Chiral two-body currents in nuclei: Gamow-Teller transitions and neutrinoless double-beta decay}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "107",
      year           = "2011",
      pages          = "062501",
      doi            = "10.1103/PhysRevLett.107.062501",
      SLACcitation   = "%%CITATION = ARXIV:1103.3622;%%"
}
      eprint         = "1103.3622",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Mikheev:1986gs,
      author         = "Mikheev, S.P. and Smirnov, A.~Y.",
      title          = "{Resonance Amplification of Oscillations in Matter and Spectroscopy of Solar Neutrinos}",
      journal        = "Sov.\ J.\ Nucl.\ Phys.",
      volume         = "42",
      pages          = "913-917",
      year           = "1985",
      SLACcitation   = "%%CITATION = SJNCA,42,913;%%",
}

@article{Minkowski:1977sc,
      author         = "Minkowski, P.",
      title          = "{$\mu \to \text{e} \gamma$ at a Rate of One Out of $10^{9}$ Muon Decays?}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "67",
      pages          = "421-428",
      doi            = "10.1016/0370-2693(77)90435-X",
      year           = "1977",
      reportNumber   = "Print-77-0182 (BERN)",
      SLACcitation   = "%%CITATION = PHLTA,B67,421;%%",
}

@article{Mitchell:1988zz,
      author         = "Mitchell, L.~W. and Fisher, Peter H.",
      title          = "{Rare decays of cadmium and tellurium}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "38",
      pages          = "895-899",
      doi            = "10.1103/PhysRevC.38.895",
      year           = "1988",
      SLACcitation   = "%%CITATION = PHRVA,C38,895;%%",
}

@article{Mitra:2011qr,
      author         = "Mitra, M. and Senjanovic, G. and Vissani, F.",
      title          = "{Neutrinoless Double Beta Decay and Heavy Sterile Neutrinos}",
      journal        = "Nucl.\ Phys.\ B",
      volume         = "856",
      pages          = "26-73",
      doi            = "10.1016/j.nuclphysb.2011.10.035",
      year           = "2012",
      SLACcitation   = "%%CITATION = ARXIV:1108.0004;%%",
}
      eprint         = "1108.0004",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Mohapatra:1979ia,
      author         = "Mohapatra, R.~N. and Senjanovic, G.",
      title          = "{Neutrino Mass and Spontaneous Parity Violation}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "44",
      pages          = "912",
      doi            = "10.1103/PhysRevLett.44.912",
      year           = "1980",
      reportNumber   = "MDDP-TR-80-060, MDDP-PP-80-105, CCNY-HEP-79-10",
      SLACcitation   = "%%CITATION = PRLTA,44,912;%%",
}

@article{Mohapatra:1980yp,
      author         = "Mohapatra, R.~N. and Senjanovic, G.",
      title          = "{Neutrino Masses and Mixings in Gauge Models with Spontaneous Parity Violation}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "23",
      pages          = "165",
      doi            = "10.1103/PhysRevD.23.165",
      year           = "1981",
      reportNumber   = "FERMILAB-PUB-80-061-THY, FERMILAB-PUB-80-061-T",
      SLACcitation   = "%%CITATION = PHRVA,D23,165;%%",
}

@article{Mohapatra:1998rq,
      author         = "Mohapatra, R.~N. and Pal, P.~B.",
      title          = "{Massive neutrinos in physics and astrophysics. (Second edition)}",
      journal        = "World Sci.\ Lect.\ Notes Phys.",
      volume         = "60",
      pages          = "1-397",
      year           = "1998",
      SLACcitation   = "%%CITATION = 00327,60,1;%%",
}

@article{Mohapatra:2006gs,
      author         = "Mohapatra, R.~N. and Smirnov, A.~Y.",
      title          = "{Neutrino Mass and New Physics}",
      journal        = "Ann.\ Rev.\ Nucl.\ Part.\ Sci.",
      volume         = "56",
      pages          = "569-628",
      doi            = "10.1146/annurev.nucl.56.080805.140534",
      year           = "2006",
      SLACcitation   = "%%CITATION = HEP-PH/0603118;%%",
}
      eprint         = "hep-ph/0603118",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Moseley:1984,
      author         = "Moseley, S.~H. and Mather, J.~C. and McCammon, D.",
      title          = "{Thermal detectors as x-ray spectrometers}",
      journal        = "J.\ Appl.\ Phys.",
      volume         = "56",
      pages          = "1257",
      doi            = "10.1063/1.334129",
      year           = "1984",
}

@article{Mott:1969nc,
		author			= {Mott, N.~F.},
		title				= "{Conduction in non-crystalline materials}",
		journal			= {Philos.\ Mag.},
		number			= {160},
		volume			= {19},
		pages				= {835-852},
		doi				= {10.1080/14786436908216338},
		year				= {1969},
}

@article{MottDavies:1980,
		author			= {Mott, N.~F. and Davies, J.~H.},
		title				= "{Metal-insulator transition in doped semiconductors}",
		journal			= {Philos.\ Mag.\ B},
		number			= {6},
		volume			= {42},
		pages				= {845-858},
		doi				= {10.1080/01418638008222332},
		year				= {1980},
}

% ------------- %
% ----- N ----- %
% ------------- %

@article{Nemevsek:2011hz,
      author         = "Nemevsek, M. and Nesti, F. and Senjanovic, G. and Zhang, Y.",
      title          = "{First Limits on Left-Right Symmetry Scale from LHC Data}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "83",
      pages          = "115014",
      doi            = "10.1103/PhysRevD.83.115014",
      year           = "2011",
      SLACcitation   = "%%CITATION = ARXIV:1103.1627;%%",
}
      eprint         = "1103.1627",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

% ------------- %
% ----- O ----- %
% ------------- %

% ------------- %
% ----- P ----- %
% ------------- %

@article{Olivieri:2017lqz,
      author         = "Olivieri, E. and Billard, J. and De Jesus, M. and
                        Juillard, A. and Leder, A.",
      title          = "{Vibrations on pulse tube based Dry Dilution
                        Refrigerators for low noise measurements}",
      journal        = "Nucl. Instrum. Meth.",
      volume         = "A858",
      year           = "2017",
      pages          = "73-79",
      doi            = "10.1016/j.nima.2017.03.045",
      eprint         = "",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1703.08957;%%"
}

@article{Pagliaroli:2010ik,
      author         = "Pagliaroli, G. and Rossi-Torres, F. and Vissani, F.",
      title          = "{Neutrino mass bound in the standard scenario for supernova electronic antineutrino emission}",
      journal        = "Astropart.\ Phys.",
      volume         = "33",
      pages          = "287-291",
      doi            = "10.1016/j.astropartphys.2010.02.007",
      year           = "2010",
      reportNumber   = "LNGS-TH-01-10",
      SLACcitation   = "%%CITATION = ARXIV:1002.3349;%%",
}
      eprint         = "1002.3349",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Palanque-Delabrouille:2013gaa,
      author         = "Palanque-Delabrouille, N. and others",
      title          = "{The one-dimensional Ly-$\alpha$ forest power spectrum from BOSS}",
      journal        = "Astron.\ Astrophys.",
      volume         = "559",
      year           = "2013",
      pages          = "A85",
      doi            = "10.1051/0004-6361/201322130",
      SLACcitation   = "%%CITATION = ARXIV:1306.5896;%%"
}
      eprint         = "1306.5896",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",

@article{Palanque-Delabrouille:2014jca,
      author         = "Palanque-Delabrouille, N. and others",
      title          = "{Constraint on neutrino masses from SDSS-III/BOSS Ly$\alpha$ forest and other cosmological probes}",
      journal        = "J.\ Cosm.\ Astropart.\ Phys.",
      volume         = "1502",
      year           = "2015",
      number         = "02",
      pages          = "045",
      doi            = "10.1088/1475-7516/2015/02/045",
      SLACcitation   = "%%CITATION = ARXIV:1410.7244;%%"
}
      eprint         = "1410.7244",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
%JCAP reference

@article{Palanque-Delabrouille:2015pga,
      author         = "Palanque-Delabrouille, N. and others",
      title          = "{Neutrino masses and cosmology with Lyman-alpha forest power spectrum}",
      journal        = "J.\ Cosm.\ Astropart.\ Phys.",
      volume         = "1511",
      year           = "2015",
      number         = "11",
      pages          = "011",
      doi            = "10.1088/1475-7516/2015/11/011",
}
      eprint         = "1506.05976",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1506.05976;%%"

@article{Pas:2015eia,
      author         = "P$\ddot{\text{a}}$s, H. and Rodejohann, W.",
      title          = "{Neutrinoless Double Beta Decay}",
      journal        = "New J.\ Phys.",
      volume         = "17",
      year           = "2015",
      number         = "11",
      pages          = "115010",
      doi            = "10.1088/1367-2630/17/11/115010",
      SLACcitation   = "%%CITATION = ARXIV:1507.00170;%%"
}
      eprint         = "1507.00170",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Pascoli:2001by,
      author         = "Pascoli, S. and Petcov, S.~T. and Wolfenstein, L.",
      title          = "{Searching for the CP violation associated with Majorana neutrinos}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "524",
      pages          = "319-331",
      doi            = "10.1016/S0370-2693(01)01403-4",
      year           = "2002",
      reportNumber   = "SISSA-81-2001-EP",
      SLACcitation   = "%%CITATION = HEP-PH/0110287;%%",
}
      eprint         = "hep-ph/0110287",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Pascoli:2003ke,
      author         = "Pascoli, S. and Petcov, S.~T.",
      title          = "{The SNO solar neutrino data, neutrinoless double beta decay and neutrino mass spectrum: Addendum}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "580",
      pages          = "280-289",
      doi            = "10.1016/j.physletb.2003.11.030",
      year           = "2004",
      reportNumber   = "SISSA-84-2003-EP, UCLA-03-TEP-26",
      SLACcitation   = "%%CITATION = HEP-PH/0310003;%%",
}
      eprint         = "hep-ph/0310003",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Pascoli:2007qh,
      author         = "Pascoli, S. and Petcov, S.~T.",
      title          = "{Majorana neutrinos, neutrino mass spectrum and the $|\left< m \right> | \sim 10^{-3}$\,eV frontier 
      						in neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "77",
      year           = "2008",
      pages          = "113003",
      doi            = "10.1103/PhysRevD.77.113003",
      reportNumber   = "SISSA-78-2007-EP, IPPP-07-83, CPT-07-166",
      SLACcitation   = "%%CITATION = ARXIV:0711.4993;%%"
}
      eprint         = "0711.4993",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Pati:1974yy,
      author         = "Pati, J.~C. and Salam, A.",
      title          = "{Lepton Number as the Fourth Color}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "10",
      pages          = "275-289",
      doi            = "10.1103/PhysRevD.10.275, 10.1103/PhysRevD.11.703.2",
      year           = "1974",
      reportNumber   = "IC-74-7",
      SLACcitation   = "%%CITATION = PHRVA,D10,275;%%",
}

@article{Perl:1975bf,
      author         = "Perl, M.~L. and others",
      title          = "{Evidence for Anomalous Lepton Production in $\el^+\,\el^-$ Annihilation}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "35",
      year           = "1975",
      pages          = "1489-1492",
      doi            = "10.1103/PhysRevLett.35.1489",
      reportNumber   = "SLAC-PUB-1626, LBL-4228",
      SLACcitation   = "%%CITATION = PRLTA,35,1489;%%"
}

@article{Petcov:2013poa,
      author         = "Petcov, S.~T.",
      title          = "{The Nature of Massive Neutrinos}",
      journal        = "Adv.\ High Energy Phys.",
      volume         = "2013",
      year           = "2013",
      pages          = "852987",
      doi            = "10.1155/2013/852987",
      SLACcitation   = "%%CITATION = ARXIV:1303.5819;%%"
}
      eprint         = "1303.5819",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Pinnarelli:1995M,
      author         = "Pinarelli, L. and Salvi, D. and Ferrara, G.",
      title          = "{The source of ancient Roman lead, as deduced from lead isotopes: the ingots from the Mal di 
      						Ventre wreck (western Sardinia, Italy)}",
      journal        = "Sci.\ Technol. Cultural Heritage",
      volume         = "4",
      year           = "1995",
      pages          = "79-86",
      url            = "http://eurekamag.com/research/020/445/020445863.php",
}

@article{Pontecorvo:1947vp,
      author         = "Pontecorvo, B.",
      title          = "{Nuclear capture of mesons and the meson decay}",
      journal        = "Phys.\ Rev.",
      volume         = "72",
      year           = "1947",
      pages          = "246-247",
      doi            = "10.1103/PhysRev.72.246",
      SLACcitation   = "%%CITATION = PHRVA,72,246;%%"
}

@article{Pontecorvo:1957cp,
      author         = "Pontecorvo, B.",
      title          = "{Mesonium and anti-mesonium}",
      journal        = "Sov.\ Phys.\ JETP",
      volume         = "6",
      pages          = "429",
      year           = "1957",
		note          = "[Zh.\ Eksp.\ Teor.\ Fiz.\ {\bf 33}, 549 (1957)]",
      SLACcitation   = "%%CITATION = SPHJA,6,429;%%",
}

@article{Pontecorvo:1959sn,
      author         = "Pontecorvo, B.",
      title          = "{Electron and Muon Neutrinos}",
      journal        = "Sov.\ Phys.\ J.\ Exp.\ Theo.\ Phys.",
      volume         = "10",
      year           = "1960",
      pages          = "1236-1240",
      note           = "[{\em Zh.\ Eksp.\ Teor.\ Fiz.\ 37, 1751(1959)}]",
      SLACcitation   = "%%CITATION = SPHJA,10,1236;%%"
}

@article{Pontecorvo:1968wp,
      author         = "Pontecorvo, B.",
      title          = "{Superweak interactions and double beta decay}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "26",
      pages          = "630-632",
      doi            = "10.1016/0370-2693(68)90437-1",
      year           = "1968",
      SLACcitation   = "%%CITATION = PHLTA,B26,630;%%",
}

@article{Prentki:1965tt,
      author         = "Prentki, J. and Veltman, M.~J.~G.",
      title          = "{Possibility of CP violation in semistrong interactions}",
      journal        = "Phys.\ Lett.",
      volume         = "15",
      pages          = "88-90",
      doi            = "10.1016/0031-9163(65)91141-8",
      year           = "1965",
      SLACcitation   = "%%CITATION = PHLTA,15,88;%%",
}

@article{Primack:1994pe,
      author         = "Primack, J.~R. and Holtzman, J. and Klypin, A. and Caldwell, D.~O.",
      title          = "{Cold + hot dark matter cosmology with $m(\nu_\mu) \approx m(\nu_\tau) \approx 2.4$\,eV}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "74",
      pages          = "2160-2163",
      doi            = "10.1103/PhysRevLett.74.2160",
      year           = "1995",
      reportNumber   = "SCIPP-94-28",
      SLACcitation   = "%%CITATION = ASTRO-PH/9411020;%%",
}
      eprint         = "astro-ph/9411020",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",

@article{Primakoff:1959,
      author         = "Primakoff, H. and Rosen, S.~P.",
      title          = "{Double beta decay}",
      journal        = "Rep.\ Prog.\ Phys.",
      volume         = "22",
      pages          = "121",
      url            = "http://stacks.iop.org/0034-4885/22/i=1/a=305",
      year           = "1959",
}

% ------------- %
% ----- Q ----- %
% ------------- %

% ------------- %
% ----- R ----- %
% ------------- %

@article{Racah:1937qq,
      author         = "Racah, G.",
      title          = "{On the symmetry of particle and antiparticle (in Italian)}",
      journal        = "Nuovo Cim.",
      volume         = "14",
      pages          = "322-328",
      doi            = "10.1007/BF02961321",
      year           = "1937",
      SLACcitation   = "%%CITATION = NUCIA,14,322;%%",
}

@article{Rahaman:2011zz,
      author         = "Rahaman, S. and Elomaa, V.~V. and Eronen, T. and Hakala, J. and Jokinen, A. and Kankainen, A. 
      					and Rissanen, J. and Suhonen, J. and Weber, C. and $\ddot{\text A}$yst$\ddot{\text o}$, J.",
      title          = "{Double-beta decay Q values of \ce{^{116}Cd} and \ce{^{130}Te}}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "703",
      pages          = "412-416",
      doi            = "10.1016/j.physletb.2011.07.078",
      year           = "2011",
      SLACcitation   = "%%CITATION = PHLTA,B703,412;%%",
}

@article{Ramond:1979py,
      author         = "Ramond, P.",
      title          = "{The Family Group in Grand Unified Theories}",
      pages          = "265-280",
      year           = "1979",
      journal        = "Conf.\ Proc.\ C79-02-25",
      volume         = "\!\!",
      eprint         = "hep-ph/9809459",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CALT-68-709",
      SLACcitation   = "%%CITATION = HEP-PH/9809459;%%",
}

@article{Ranitzsch:2012,
      author         = "Ranitzsch, P.~C.~O. and Porst, J.~P. and Kempf, S. and Pies, C. and Schafer, S. and Hengstler, D. 
      						and Fleischmann, A. and Enss, C. and Gastaldo, L.",
      title          = "{Development of Metallic Magnetic Calorimeters for High Precision Measurements of 
      						Calorimetric \ce{^{187}Re} and \ce{^{163}Ho} Spectra}",
      journal        = "J.\ Low Temp.\ Phys.",
      volume         = "167",
      pages          = "1004-1014",
      doi            = "10.1007/s10909-012-0556-0",
      year           = "2012",
}

@article{Rath:2010zz,
      author         = "Rath, P.~K. and Chandra, R. and Chaturvedi, K. and Raina, P.~K. and Hirsch, J.~G.",
      title          = "{Uncertainties in nuclear transition matrix elements for
                        neutrinoless $\beta \beta $ decay within the PHFB model}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "82",
      year           = "2010",
      pages          = "064310",
      doi            = "10.1103/PhysRevC.82.064310",
      SLACcitation   = "%%CITATION = ARXIV:1104.3965;%%"
}
      eprint         = "1104.3965",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Rath:2013fma,
      author         = "Rath, P.~K. and Chandra, R. and Chaturvedi, K. and Lohani, P. and Raina, P. K. and Hirsch, J.~G.",
      title          = "{Neutrinoless $\beta\beta$ decay transition matrix elements within mechanisms involving light 
      						Majorana neutrinos, classical Majorons, and sterile neutrinos}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "88",
      year           = "2013",
      number         = "6",
      pages          = "064322",
      doi            = "10.1103/PhysRevC.88.064322",
      SLACcitation   = "%%CITATION = ARXIV:1308.0460;%%"
}
      eprint         = "1308.0460",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Redshaw:2009zz,
      author         = "Redshaw, M. and Mount, B.~J. and Myers, E.G. and Avignone, F.~T.",
      title          = "{Masses of Te-130 and Xe-130 and Double-beta-Decay Q Value of Te-130}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "102",
      pages          = "212502",
      doi            = "10.1103/PhysRevLett.102.212502",
      year           = "2009",
      SLACcitation   = "%%CITATION = PRLTA,102,212502;%%",
}

@article{Reines:1953kf,
      author         = "Reines, F. and Cowan, C.L.",
      title          = "{A Proposed experiment to detect the free neutrino}",
      journal        = "Phys.\ Rev.",
      volume         = "90",
      year           = "1953",
      pages          = "492-493",
      doi            = "10.1103/PhysRev.90.492",
      SLACcitation   = "%%CITATION = PHRVA,90,492;%%"
}

@article{Reines:1953pu,
      author         = "Reines, F. and Cowan, C.~L.",
      title          = "{Detection of the free neutrino}",
      journal        = "Phys. Rev.",
      volume         = "92",
      year           = "1953",
      pages          = "830-831",
      doi            = "10.1103/PhysRev.92.830",
      SLACcitation   = "%%CITATION = PHRVA,92,830;%%"
}

@article{Reines:1960pr,
      author         = "Reines, F. and Cowan, C.~L. and Harrison, F.~B. and McGuire, A.~D. and Kruse, H.~W.",
      title          = "{Detection of the free anti-neutrino}",
      journal        = "Phys.\ Rev.",
      volume         = "117",
      year           = "1960",
      pages          = "159-173",
      doi            = "10.1103/PhysRev.117.159",
      SLACcitation   = "%%CITATION = PHRVA,117,159;%%"
}

@article{Robertson:2013cy,
      author         = "Robertson, R.~G.~H.",
      title          = "{Empirical Survey of Neutrinoless Double Beta Decay Matrix Elements}",
      journal        = "Mod.\ Phys.\ Lett.\ A",
      volume         = "28",
      pages          = "1350021",
      doi            = "10.1142/S0217732313500211",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1301.1323;%%",
}
      eprint         = "1301.1323",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Rochester:1947mi,
      author         = "Rochester, G.~D. and Butler, C.~C.",
      title          = "{Evidence for the Existence of New Unstable Elementary Particles}",
      journal        = "Nature",
      volume         = "160",
      year           = "1947",
      pages          = "855-857",
      doi            = "10.1038/160855a0",
      SLACcitation   = "%%CITATION = NATUA,160,855;%%"
}
%kaon meson observation

@article{Rodejohann:2011a,
      author         = "Rodejohann, W.",
      title          = "{Neutrinoless-double beta decay and particle physics}",
      journal        = "Int.\ J.\ Mod.\ Phys.\ E",
      volume         = "20",
      year           = "2011",
      pages          = "1833-1930",
      doi            = "10.1142/S0218301311020186",
}
      eprint         = "1106.1334",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Rodejohann:2012xd,
      author         = "Rodejohann, W.",
      title          = "{Neutrinoless double beta decay and neutrino physics}",
      journal        = "J.\ Phys.\ G",
      volume         = "39",
      year           = "2012",
      pages          = "124008",
      doi            = "10.1088/0954-3899/39/12/124008",
      SLACcitation   = "%%CITATION = ARXIV:1206.2560;%%"
}
      eprint         = "1206.2560",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Rodin:2003eb,
      author         = "Rodin, V.~A. and Faessler, A. and \u{S}imkovic, F. and Vogel, P.",
      title          = "{On the uncertainty in the $0\nu\beta\beta$ decay nuclear matrix elements}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "68",
      pages          = "044302",
      doi            = "10.1103/PhysRevC.68.044302",
      year           = "2003",
      SLACcitation   = "%%CITATION = NUCL-TH/0305005;%%",
}
      eprint         = "nucl-th/0305005",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Rodin:2006yk,
      author         = "Rodin, V.~A. and Faessler, A. and \u{S}imkovic, F. and Vogel, P.",
      title          = "{Assessment of uncertainties in QRPA $0\nu\beta\beta$ nuclear matrix elements}",
      journal        = "Nucl.\ Phys.\ A",
      volume         = "766",
      pages          = "107-131",
      doi            = "10.1016/j.nuclphysa.2005.12.004",
      year           = "2006",
      SLACcitation   = "%%CITATION = ARXIV:0706.4304;%%",
}
      eprint         = "0706.4304",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Rodriguez:2010mn,
      author         = "Rodriguez, T.~R. and Martinez-Pinedo, G.",
      title          = "{Energy density functional study of nuclear matrix elements for neutrinoless $\beta\beta$ decay}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "105",
      year           = "2010",
      pages          = "252503",
      doi            = "10.1103/PhysRevLett.105.252503",
      SLACcitation   = "%%CITATION = ARXIV:1008.5260;%%"
}
      eprint         = "1008.5260",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Rontegen:1896NA,
      author         = "R$\ddot{\text o}$ntgen, W.~C.",
      title          = "{On a New Kind of Rays}",
      journal        = "Nature",
      volume         = "53",
      year           = "1896",
      pages          = "274-276",
      doi				= "10.1038/053274b0",
      note				= "[Original work in: 
      					{\em Sitzungsberichte der W$\ddot{\text u}$rzburger Physik.-medic. Gesellschaft} (1895)]",
}

@article{Rutherford:1899NA,
      author         = "Rutherford, E.",
      title          = "{Uranium radiation and the electrical conduction produced by it}",
      journal        = "Phil.\ Mag.",
      volume         = "47",
      year           = "1899",
      pages          = "109-163",
      doi				= "10.1080/14786449908621245",
}
      series			= "5",
      number			= "284",


@article{Rutherford:1903NA,
      author         = "Rutherford, E.",
      title          = "{The magnetic and electric deviation of the easily absorbed rays from radium}",
      journal        = "Phil.\ Mag.",
      volume         = "5",
      year           = "1903",
      pages          = "177-187",
      doi				= "10.1080/14786440309462912",
}
      series			= "6",
      number			= "26",

@article{Rutherford:1929NA,
      author         = "Rutherford, E. and Chadwick, J.",
      title          = "{Energy Relations in Artificial Disintegration}",
      journal        = "Math.\ Proc.\ Cambridge Phil.\ Soc.",
      volume         = "25",
      year           = "1929",
      pages          = "186-192",
      doi				= "10.1017/S0305004100018703",
}

% ------------- %
% ----- S ----- %
% ------------- %

@article{Saakyan:2013yna,
      author         = "Saakyan, R.",
      title          = "{Two-Neutrino Double-Beta Decay}",
      journal        = "Ann.\ Rev.\ Nucl.\ Part.\ Sci.",
      volume         = "63",
      pages          = "503-529",
      doi            = "10.1146/annurev-nucl-102711-094904",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARNUA,63,503;%%",
}

@article{Salam:1957st,
      author         = "Salam, A.",
      title          = "{On parity conservation and neutrino mass}",
      journal        = "Nuovo Cim.",
      volume         = "5",
      pages          = "299-301",
      doi            = "10.1007/BF02812841",
      year           = "1957",
      SLACcitation   = "%%CITATION = NUCIA,5,299;%%",
}

@article{Sakharov:1967dj,
      author         = "Sakharov, A.~D.",
      title          = "{Violation of CP Invariance, c Asymmetry, and Baryon Asymmetry of the Universe}",
      journal        = "Pisma Zh.\ Eksp.\ Teor.\ Fiz.",
      volume         = "5",
      pages          = "32-35",
      url            = "http://iopscience.iop.org/article/10.1070/PU1991v034n05ABEH002497/meta;
      						jsessionid=66AF62A9E1943AE2989F9A561A276B1D.c4.iopscience.cld.iop.org",
      year           = "1967",
      SLACcitation   = "%%CITATION = ZFPRA,5,32;%%",
}
      doi            = "10.1070/PU1991v034n05ABEH002497",

@article{Schechter:1981bd,
      author         = "Schechter, J. and Valle, J.~W.~F.",
      title          = "{Neutrinoless Double beta Decay in $SU(2) \times U(1)$ Theories}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "25",
      pages          = "2951",
      doi            = "10.1103/PhysRevD.25.2951",
      year           = "1982",
      reportNumber   = "SU-4217-213, COO-3533-213",
      SLACcitation   = "%%CITATION = PHRVA,D25,2951;%%",
}

@article{Schwark&al:1983,
		author        	= "Schwark, M. and Pobell, F. and Halperin, W.~P. and Buchal, C. and Hanssen, J. and 
								Kubota, M. and Mueller, R.~M.",
		title				= "{Ortho-para conversion of hydrogen in copper as origin of time-dependent heat leaks}",
		journal			= "J.\ Low Temp.\ Phys.",
		volume			= "53",
		pages				= "685-694",
		doi				= "10.1007/BF00684000",
		year				= "1983"
}
		issn				= {0022-2291},
		number			= {5-6},
		url				= {http://dx.doi.org/10.1007/BF00684000},
		publisher		= {Kluwer Academic Publishers-Plenum Publishers},

@article{Schwingenheuer:2012zs,
      author         = "Schwingenheuer, B.",
      title          = "{Status and prospects of searches for neutrinoless double beta decay}",
      journal        = "Ann.\ Phys.",
      volume         = "525",
      year           = "2013",
      pages          = "269-280",
      doi            = "10.1002/andp.201200222",
      SLACcitation   = "%%CITATION = ARXIV:1210.7432;%%"
}
      eprint         = "1210.7432",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Scielzo:2009nh,
      author         = "Scielzo, N.~D. and others",
      title          = "{Double-beta decay Q values of Te-13-, Te-128, and Te-120}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "80",
      pages          = "025501",
      doi            = "10.1103/PhysRevC.80.025501",
      year           = "2009",
      SLACcitation   = "%%CITATION = ARXIV:0902.2376;%%",
}
      eprint         = "0902.2376",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",

@article{Shimizu:1974,
      author         = "Shimizu, K. and Ichimura, M. and Arima, A.",
      title          = "{Magnetic moments and GT-type β-decay matrix elements in nuclei with a $LS$ doubly closed 
      						shell plus or minus one nucleon}",
      journal        = "Nucl.\ Phys.\ A",
      volume         = "226",
      year           = "1974",
      pages          = "282-318",
      doi            = "10.1016/0375-9474(74)90407-2",
}

@article{Simkovic:1999re,
      author         = "\u{S}imkovic, F. and Pantis, G. and Vergados, J.~D. and Faessler, A.",
      title          = "{Additional nucleon current contributions to neutrinoless double beta decay}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "60",
      year           = "1999",
      pages          = "055502",
      doi            = "10.1103/PhysRevC.60.055502",
      SLACcitation   = "%%CITATION = HEP-PH/9905509;%%"
}
      eprint         = "hep-ph/9905509",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Simkovic:2010ka,
      author         = "\u{S}imkovic, F. and Vergados, J. and Faessler, A.",
      title          = "{Few active mechanisms of the neutrinoless double beta-decay and effective mass of 
      						Majorana neutrinos}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "82",
      pages          = "113015",
      doi            = "10.1103/PhysRevD.82.113015",
      year           = "2010",
      SLACcitation   = "%%CITATION = ARXIV:1006.0571;%%",
}
      eprint         = "1006.0571",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Simkovic:2012hq,
      author         = "\u{S}imkovic, F. and Bilenky, S.~M. and Faessler, A. and Gutsche, T.",
      title          = "{Possibility of measuring the CP Majorana phases in $0\nu\beta\beta$ decay}",
      journal        = "Phys.\ Rev.\ D",
      number         = "7",
      volume         = "87",
      pages          = "073002",
      doi            = "10.1103/PhysRevD.87.073002",
      year           = "2013",
      SLACcitation   = "%%CITATION = ARXIV:1210.1306;%%",
}
      eprint         = "1210.1306",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Simkovic:2013qiy,
      author         = "\u{S}imkovic, F. and Rodin, V. and Faessler, A. and Vogel, P.",
      title          = "{$0\nu\beta\beta$ and $2\nu\beta\beta$ nuclear matrix elements, quasiparticle random-phase 
      						approximation, and isospin symmetry restoration}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "87",
      year           = "2013",
      number         = "4",
      pages          = "045501",
      doi            = "10.1103/PhysRevC.87.045501",
      reportNumber   = "CALT-68-2909",
      SLACcitation   = "%%CITATION = ARXIV:1302.1509;%%"
}
      eprint         = "1302.1509",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Simon:1935,
      author         = "Simon, F.",
      title          = "{Application of Low Temperature Calorimetry to Radioactive Measurements}",
      journal        = "Nature",
      volume         = "135",
      pages          = "763",
      doi            = "10.1038/135763a0",
      year           = "1935",
}

@article{Soddy:1913M,
      author         = "Soddy, F.",
      title          = "{The Radio-Elements and the Periodic Law}",
      journal        = "Chem.\ News",
      volume         = "107",
      year           = "1913",
      pages          = "97-99",
}

@article{Stefanik:2015twa,
      author         = "\u{S}tef\'anik, D. and Dvornick\'y, R. and \u{S}imkovic, F. and Vogel, P.",
      title          = "{Reexamining the light neutrino exchange mechanism of the $0\nu\beta\beta$ decay with left- and 
      						right-handed leptonic and hadronic currents}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "92",
      year           = "2015",
      number         = "5",
      pages          = "055502",
      doi            = "10.1103/PhysRevC.92.055502",
      SLACcitation   = "%%CITATION = ARXIV:1506.07145;%%"
}
      eprint         = "1506.07145",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Stoica:2013lka,
      author         = "Stoica, S. and Mirea, M.",
      title          = "{New calculations for phase space factors involved in double-$\beta$ decay}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "88",
      year           = "2013",
      number         = "3",
      pages          = "037303",
      doi            = "10.1103/PhysRevC.88.037303",
      SLACcitation   = "%%CITATION = ARXIV:1307.0290;%%"
}
      eprint         = "1307.0290",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

@article{Sudarshan:1958vf,
      author         = "Sudarshan, E.~C.~G. and Marshak, R.~E.",
      title          = "{Chirality invariance and the universal Fermi interaction}",
      journal        = "Phys.\ Rev.",
      volume         = "109",
      year           = "1958",
      pages          = "1860-1860",
      doi            = "10.1103/PhysRev.109.1860.2",
      SLACcitation   = "%%CITATION = PHRVA,109,1860;%%"
}

@article{Suhonen:2013laa,
      author         = "Suhonen, J. and Civitarese, O.",
      title          = "{Probing the quenching of $g_A$ by single and double beta decays}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "725",
      year           = "2013",
      pages          = "153-157",
      doi            = "10.1016/j.physletb.2013.06.042",
      SLACcitation   = "%%CITATION = PHLTA,B725,153;%%"
}

% ------------- %
% ----- T ----- %
% ------------- %

@article{Tello:2010am,
      author         = "Tello, V. and Nemevsek, M. and Nesti, F. and Senjanovic, G. and Vissani, F.",
      title          = "{Left-Right Symmetry: from LHC to Neutrinoless Double Beta Decay}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "106",
      pages          = "151801",
      doi            = "10.1103/PhysRevLett.106.151801",
      year           = "2011",
      SLACcitation   = "%%CITATION = ARXIV:1011.3522;%%",
}
      eprint         = "1011.3522",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{'tHooft:1976up,
      author         = "'t Hooft, G.",
      title          = "{Symmetry Breaking Through Bell-Jackiw Anomalies}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "37",
      pages          = "8-11",
      doi            = "10.1103/PhysRevLett.37.8",
      year           = "1976",
      reportNumber   = "PRINT-76-0254 (HARVARD)",
      SLACcitation   = "%%CITATION = PRLTA,37,8;%%",
}

@article{Tomoda:1990rs,
      author         = "Tomoda, T.",
      title          = "{Double beta decay}",
      journal        = "Rep.\ Prog.\ Phys.",
      volume         = "54",
      year           = "1991",
      pages          = "53-126",
      doi            = "10.1088/0034-4885/54/1/002",
      reportNumber   = "PSI-PR-90-20",
      SLACcitation   = "%%CITATION = RPPHA,54,53;%%"
}

@article{Tretyak:2002dx,
      author         = "Tretyak, V.~I. and Zdesenko, Y.~G.",
      title          = "{Tables of double beta decay data: An update}",
      journal        = "Atom.\ Data Nucl.\ Data Tabl.",
      volume         = "80",
      year           = "2002",
      pages          = "83-116",
      doi            = "10.1006/adnd.2001.0873",
      SLACcitation   = "%%CITATION = ADNDA,80,83;%%"
}

@article{Trincherini:2009M,
      author         = "Trincherini, P.~R. and Domergue, C. and Manteca, I. and Nesta, A. and Quarati, P.",
      title          = "{The identification of lead ingots from the Roman mines of Cartagena (Murcia, Spain): 
      						the role of lead isotope analysis}",
      journal        = "J.\ Roman Archaeology",
      volume         = "22",
      year           = "2009",
      pages          = "123-145",
      url            = "http://www.journalofromanarch.com/v22_thum_page.html",
}
      eprint         = "1002.3557",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.soc-ph",

% ------------- %
% ----- U ----- %
% ------------- %

% ------------- %
% ----- V ----- %
% ------------- %

@article{Vanzini:2001rx,
      author         = "Vanzini, M. and others",
      title          = "{High-resolution bolometers for rare events detection}",
      journal        = "Nucl.\ Instrum.\ Meth.\ A",
      volume         = "461",
      year           = "2001",
      pages          = "293-296",
      doi            = "10.1016/S0168-9002(00)01228-6",
}
      booktitle      = "{Frontier detectors for frontier physics. Proceedings, 8th Pisa Meeting on Advanced Detectors: 
      						La Biodola, Italy, May 21-27, 2000}",
      SLACcitation   = "%%CITATION = NUIMA,A461,293;%%"

@article{Vergados:2012xy,
      author         = "Vergados, J.~D. and Ejiri, H. and \u{S}imkovic, F.",
      title          = "{Theory of Neutrinoless Double Beta Decay}",
      journal        = "Rep.\ Prog.\ Phys.",
      volume         = "75",
      year           = "2012",
      pages          = "106301",
      doi            = "10.1088/0034-4885/75/10/106301",
      SLACcitation   = "%%CITATION = ARXIV:1205.0649;%%"
}
      eprint         = "1205.0649",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Vissani:1999tu,
      author         = "Vissani, F.",
      title          = "{Signal of neutrinoless double beta decay, neutrino spectrum and oscillation scenarios}",
      journal        = "J.\ High Energy Phys.",
      volume         = "9906",
      pages          = "022",
      doi            = "10.1088/1126-6708/1999/06/022",
      year           = "1999",
      SLACcitation   = "%%CITATION = HEP-PH/9906525;%%",
}
      eprint         = "hep-ph/9906525",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Vissani:2001im,
      author         = "Vissani, F.",
      title          = "{Expected properties of massive neutrinos for mass matrices with a dominant block and random 
      						coefficients order unity}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "508",
      year           = "2001",
      pages          = "79-84",
      doi            = "10.1016/S0370-2693(01)00485-3",
      SLACcitation   = "%%CITATION = HEP-PH/0102236;%%"
}
      eprint         = "hep-ph/0102236",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Vissani:2003aj,
      author         = "Vissani, F. and Narayan, M. and Berezinsky, V.",
      title          = "{$U_{e3}$ from physics above the GUT scale}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "571",
      year           = "2003",
      pages          = "209-216",
      doi            = "10.1016/j.physletb.2003.07.002",
      SLACcitation   = "%%CITATION = HEP-PH/0305233;%%"
}
      eprint         = "hep-ph/0305233",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",

@article{Vogel:2012ja,
      author         = "Vogel, P.",
      title          = "{Nuclear structure and double beta decay}",
      journal        = "J.\ Phys.\ G",
      volume         = "39",
      year           = "2012",
      pages          = "124002",
      doi            = "10.1088/0954-3899/39/12/124002",
      SLACcitation   = "%%CITATION = ARXIV:1208.1992;%%"
}
      eprint         = "1208.1992",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",

% ------------- %
% ----- W ----- %
% ------------- %

@article{Weinberg:1962zza,
      author         = "Weinberg, S.",
      title          = "{Universal Neutrino Degeneracy}",
      journal        = "Phys.\ Rev.",
      volume         = "128",
      pages          = "1457-1473",
      doi            = "10.1103/PhysRev.128.1457",
      year           = "1962",
      SLACcitation   = "%%CITATION = PHRVA,128,1457;%%",
}

@article{Weinberg:1967tq,
      author         = "Weinberg, S.",
      title          = "{A Model of Leptons}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "19",
      pages          = "1264-1266",
      doi            = "10.1103/PhysRevLett.19.1264",
      year           = "1967",
      SLACcitation   = "%%CITATION = PRLTA,19,1264;%%",
}

@article{Weinberg:1979sa,
      author         = "Weinberg, S.",
      title          = "{Baryon and Lepton Nonconserving Processes}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "43",
      pages          = "1566-1570",
      doi            = "10.1103/PhysRevLett.43.1566",
      year           = "1979",
      reportNumber   = "HUTP-79-A050",
      SLACcitation   = "%%CITATION = PRLTA,43,1566;%%",
}

@article{Weinberg:1981wj,
      author         = "Weinberg, S.",
      title          = "{Supersymmetry at Ordinary Energies. 1. Masses and Conservation Laws}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "26",
      year           = "1982",
      pages          = "287",
      doi            = "10.1103/PhysRevD.26.287",
      reportNumber   = "HUTP-81-A047",
      SLACcitation   = "%%CITATION = PHRVA,D26,287;%%"
}

@article{Weyl:1929fm,
      author         = "Weyl, H.",
      title          = "{Electron and Gravitation. 1. (in German)}",
      journal        = "Z.\ Phys.",
      volume         = "56",
      pages          = "330-352",
      doi            = "10.1007/BF01339504",
      year           = "1929",
      SLACcitation   = "%%CITATION = ZEPYA,56,330;%%",
}

@article{White:1990,
      author         = "White, G.~K. and Collocott, S.J. and Collins, J.~G.",
      title          = "{Thermal properties of paratellurite (\ce{TeO_2}) at low temperatures }",
      journal        = "J.\ Phys. Condensed Matter",
      number         = "37",
      volume         = "2",
      pages          = "7715",
      url            = "http://stacks.iop.org/0953-8984/2/i=37/a=015",
      year           = "1990",
}

@article{Wilczek:1979hc,
      author         = "Wilczek, F. and Zee, A.",
      title          = "{Operator Analysis of Nucleon Decay}",
      journal        = "Phys.\ Rev.\ Lett.",
      volume         = "43",
      pages          = "1571-1573",
      doi            = "10.1103/PhysRevLett.43.1571",
      year           = "1979",
      reportNumber   = "Print-79-0709 (PRINCETON)",
      SLACcitation   = "%%CITATION = PRLTA,43,1571;%%",
}

@article{Wilkinson:1973zz,
      author         = "Wilkinson, D.~H.",
      title          = "{Renormalization of the Axial-Vector Coupling Constant in Nuclear beta Decay}",
      journal        = "Phys.\ Rev.\ C",
      volume         = "7",
      year           = "1973",
      pages          = "930-936",
      doi            = "10.1103/PhysRevC.7.930",
      SLACcitation   = "%%CITATION = PHRVA,C7,930;%%"
}

@article{Wilkinson:1973_2,
      author         = "Wilkinson, D.~H.",
      title          = "{Renormalization of the axial-vector coupling constant in nuclear $\beta$-decay (II)}",
      journal        = "Nucl.\ Phys.\ A",
      volume         = "209",
      year           = "1973",
      pages          = "470-484",
      doi            = "10.1016/0375-9474(73)90840-3",
}

@article{Wilkinson:1974,
      author         = "Wilkinson, D.~H.",
      title          = "{Renormalization of the axial-vector coupling constant in nuclear $\beta$-decay (III)}",
      journal        = "Nucl.\ Phys.\ A",
      volume         = "225",
      year           = "1974",
      pages          = "365-381",
      doi            = "10.1016/0375-9474(74)90347-9",
}

@article{Wolfenstein:1977ue,
      author         = "Wolfenstein, L.",
      title          = "{Neutrino Oscillations in Matter}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "17",
      pages          = "2369-2374",
      doi            = "10.1103/PhysRevD.17.2369",
      year           = "1978",
      reportNumber   = "COO-3066-102",
      SLACcitation   = "%%CITATION = PHRVA,D17,2369;%%",
}

@article{Wong:2011ip,
      author         = "Wong, Y.~Y.~Y.",
      title          = "{Neutrino mass in cosmology: status and prospects}",
      journal        = "Ann.\ Rev.\ Nucl.\ Part.\ Sci.",
      volume         = "61",
      year           = "2011",
      pages          = "69-98",
      doi            = "10.1146/annurev-nucl-102010-130252",
      reportNumber   = "TTK-11-56",
      SLACcitation   = "%%CITATION = ARXIV:1111.1436;%%"
}
      eprint         = "1111.1436",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",

@article{Wu:1957my,
      author         = "Wu, C.~S. and Ambler, E. and Hayward, R.~W. and Hoppes, D.~D. and Hudson, R.~P.",
      title          = "{Experimental Test of Parity Conservation in Beta Decay}",
      journal        = "Phys.\ Rev.",
      volume         = "105",
      year           = "1957",
      pages          = "1413-1414",
      doi            = "10.1103/PhysRev.105.1413",
      SLACcitation   = "%%CITATION = PHRVA,105,1413;%%"
}

@article{Wulandari:2003cr,
      author         = "Wulandari, H. and Jochum, J. and Rau, W. and von Feilitzsch, F.",
      title          = "{Neutron flux at the Gran Sasso underground laboratory revisited}",
      journal        = "Astropart.\ Phys.",
      volume         = "22",
      year           = "2004",
      pages          = "313-322",
      doi            = "10.1016/j.astropartphys.2004.07.005",
}
      eprint         = "hep-ex/0312050",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = HEP-EX/0312050;%%"

@article{Wyman:2013lza,
      author         = "Wyman, M. and Rudd, D.~H. and Vanderveld, R.~A. and Hu, W.",
      title          = "{Neutrinos Help Reconcile Planck Measurements with the Local Universe}",
      journal        = "Phys.\ Rev.\ Lett.",
      number         = "5",
      volume         = "112",
      pages          = "051302",
      doi            = "10.1103/PhysRevLett.112.051302",
      year           = "2014",
      SLACcitation   = "%%CITATION = ARXIV:1307.7715;%%",
}
      eprint         = "1307.7715",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",

% ------------- %
% ----- X ----- %
% ------------- %

@article{Xu:2005sc,
		author 			= "Xu, R. and Xu, L.",
		title 			= "An experimental investigation of thermal contact conductance of stainless steel at low temperatures ",
		journal 			= "Cryogenics",
		volume 			= "45",
		number 			= "10–11",
		pages 			= "694 - 704",
		year 				= "2005",
		issn 				= "0011-2275",
		doi 				= "10.1016/j.cryogenics.2005.09.002",
}
		url 				= "http://www.sciencedirect.com/science/article/pii/S0011227505001086"

% ------------- %
% ----- Y ----- %
% ------------- %

% ------------- %
% ----- Z ----- %
% ------------- %

@article{Zdesenko:1980,
      author         = "Zdesenko, Y.~G.",
      title          = "{On lepton charge conservation in the double $\beta$ decay of \ce{^{130}Te}}",
      journal        = "JETP Lett.",
      volume         = "32",
      pages          = "58",
      url            = "http://www.jetpletters.ac.ru/ps/1423/article_21633.shtml",
      year           = "1980",
}

@article{Zdesenko:2002kz,
      author         = "Zdesenko, Y.~G. and Danevich, F.~A. and Tretyak, V.~I.",
      title          = "{Has neutrinoless double beta decay of Ge-76 been really observed?}",
      journal        = "Phys.\ Lett.\ B",
      volume         = "546",
      year           = "2002",
      pages          = "206-215",
      doi            = "10.1016/S0370-2693(02)02705-3",
      SLACcitation   = "%%CITATION = PHLTA,B546,206;%%"
}

@article{Zeldovich:1981wf,
      author         = "Zel'dovich, Y.~B. and Khlopov, M.~Y.",
      title          = "{The Neutrino Mass in Elementary Particle Physics and in Big Bang Cosmology}",
      journal        = "Sov.\ Phys.\ Usp.",
      volume         = "24",
      pages          = "755-774",
      doi            = "10.1070/PU1981v024n09ABEH004816",
      year           = "1981",
      SLACcitation   = "%%CITATION = SOPUA,24,755;%%",
}

@article{Zhang:2015uhk,
      author         = "Zhang, X.",
      title          = "{Impacts of dark energy on weighing neutrinos after Planck 2015}",
      journal        = "Phys.\ Rev.\ D",
      volume         = "93",
      year           = "2016",
      number         = "8",
      pages          = "083011",
      doi            = "10.1103/PhysRevD.93.083011",
}
      eprint         = "1511.02651",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1511.02651;%%"



==> ref_Proceedings.tex <==
@article{Alessandrello:1992jc,
      author         = "Alessandrello, A. and others",
      title          = "{A search for neutrinoless double beta decay of \ce{^{130}Te} with a bolometric detector}",
      journal        = "Nucl.\ Phys.\ B (Proc.\ Suppl.)",
      volume         = "28\,A",
      pages          = "229-232",
      doi            = "10.1016/0920-5632(92)90177-T",
      year           = "1992",
      SLACcitation   = "%%CITATION = NUPHZ,28A,229;%%",
}

@article{Alessandrello:1994_XX,
      author         = "Giuliani, A. and others",
      title          = "{The Milano-Gran Sasso experiment on double beta decay using thermal dettectors}",
      journal        = "Proc.\ 27th Int.\ Conf.\ on High-energy Phys.",
      pages          = "943-944",
      year           = "1994",
      SLACcitation   = "%%CITATION = CONFP,C910725V1,670;%%",
}
      journal        = "Conf.\ Proc.\ C94-07-20",

@article{Alessandrello:1989bu,
      author         = "Alessandrello, A. and Brofferio, C. and Camin, D.~V. and
                        Cremonesi, O. and Fiorini, E. and Giuliani, A. and Pessina, G. and Previtali, E.",
      title          = "{The first underground low radioactivity bolometric system}",
      journal        = "Proc.\ 3rd Int.\ Workshop on Low Temp.\ Det.\ for Neutrinos and Dark Matter",
      pages          = "253-262",
      year           = "1989",
      SLACcitation   = "%%CITATION = INSPIRE-293097;%%",
}
      journal        = "Conf.\ Proc.\ C89-09-20",

@article{Asakura:2014lma,
      author         = "Asakura, K. and others",
      title          = "{Results from KamLAND-Zen}",
      collaboration  = "KamLAND-Zen Collaboration",
      journal        = "AIP Conf.\ Proc.",
      volume         = "1666",
      year           = "2015",
      pages          = "170003",
      doi            = "10.1063/1.4915593",
}
      booktitle      = "{Proceedings, 26th International Conference on Neutrino
                        Physics and Astrophysics (Neutrino 2014): Boston,
                        Massachusetts, United States, June 2-7, 2014}",
      eprint         = "1409.0077",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1409.0077;%%"

@article{Brofferio:1995wx,
      author         = "Brofferio, C. and others",
      title          = "{Improvements in Te-130 double beta decay search with cryogenic TeO-2 array detectors}",
      journal        = "Nucl.\ Phys.\ B (Proc.\ Suppl.)",
      volume         = "48",
      pages          = "238-240",
      doi            = "10.1016/0920-5632(96)00249-6",
      year           = "1996",
      SLACcitation   = "%%CITATION = NUPHZ,48,238;%%",
}

@article{Croce:2015kwa,
      author         = "Croce, M.~P. and others",
      title          = "{Development of holmium-163 electron-capture spectroscopy with transition-edge sensors}",
      journal        = "J.\ Low.\ Temp.\ Phys.",
      volume         = "184",
      year           = "2016",
      number         = "3-4",
      pages          = "958-968",
      doi            = "10.1007/s10909-015-1451-2",
}
      booktitle      = "{Proceedings, 16th International Workshop on Low Temperature Detectors (LTD 16): Grenoble, France, 
      						July 20-24, 2016}",
      eprint         = "1510.03874",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      reportNumber   = "LOS-ALAMOS-NATIONAL-LABORATORY-REPORT-LA-UR-15-27688, APPROVED-FOR --UNLIMITED-RELEASE",
      SLACcitation   = "%%CITATION = ARXIV:1510.03874;%%"

@article{Das:1965M,
      author         = "Das, P. and De Bruyn Ouboter, R. and Taconis, K.~W.",
      journal        = "Proc.\ 9th Int.\ Conf.\ Low Temp.\ Phys.",
      year           = "1965",
      pages          = "1253",
}

@article{Engert:2012NT,
      author         = "Engert, J. and Heyer, D. and Beyer, J. and Barthelmess, H.~J.",
      title          = "{Noise thermometry at low temperatures: MFFT measurements between 1.6\,K and 1\,mK}",
      journal        = "J.\ Phys.\ Conf.\ Ser.",
      volume         = "400",
      year           = "2012",
      pages          = "05203",
      doi            = "10.1088/1742-6596/400/5/052003",
}

@article{Gastaldo:2013wha,
      author         = "Gastaldo, L. and others",
      title          = "{The Electron Capture \ce{^{163}Ho} Experiment ECHo: an overview}",
      journal        = "J.\ Low Temp.\ Phys.",
      volume         = "176",
      year           = "2014",
      number         = "5-6",
      pages          = "876-884",
      doi            = "10.1007/s10909-014-1187-4",
}
      booktitle      = "{Proceedings, 15th International Workshop on Low Temperature Detectors (LTD-15): Pasadena, 
      						California, June 24-28, 2013}",
      eprint         = "1309.5214",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1309.5214;%%"

@article{Giuliani:1991ze,
      author         = "Giuliani, A. and others",
      title          = "{A low temperature \ce{TeO_2} detector to search for double beta decay of \ce{^{130}Te}}",
      journal        = "Proc.\ Joint Int.\ Lepton Photon Symposium at High Energies (15th) and European 
      					Phys.\ Soc.\ Conf.\ on High-energy Phys.",
      pages          = "670-672",
      year           = "1991",
      SLACcitation   = "%%CITATION = CONFP,C910725V1,670;%%",
}
      journal        = "Conf.\ Proc.\ C91-07-25",

@article{Gomez-Cadenas:2015twa,
      author         = "G\'{o}mez-Cadenas, J.~J. and Mart\`in-Albo, J.",
      title          = "{Phenomenology of neutrinoless double beta decay}",
      journal        = "Proc.\ of Science",
      volume         = "(GSSI14)",
      year           = "2015",
      pages          = "004",
      url				= "http://pos.sissa.it/cgi-bin/reader/conf.cgi?confid=229",
      SLACcitation   = "%%CITATION = ARXIV:1502.00581;%%"
}
      booktitle      = "{Proceedings, Gran Sasso Summer Institute 2014: Hands-On
                        Experimental Underground Physics at LNGS}",
      eprint         = "1502.00581",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",

@article{Langley:1881,
      author         = "Langley, S.~P.",
      title          = "{The Bolometer and Radiant Energy}",
      journal        = "Proc.\ Am.\ Acad.\ Arts Sci.\ XVI",
      pages          = "342",
      year           = "1881",
}

@article{London:1951M,
      author         = "London, H.",
      journal        = "Proc.\ 2nd Int.\ Conf.\ on Low Temp.\ Phys.",
      year           = "1951",
      pages          = "157",
}

@article{Marcocci:2015uia,
      author         = "Marcocci, S. and Piastra, F. and Gorla, P.",
      title          = "{Hands on CUORE: investigation on the vibrations and temperature control of the cryostat}",
      journal        = "Proc.\ of Science",
      volume         = "(GSSI14)",
      year           = "2015",
      pages          = "023",
      url				= "http://pos.sissa.it/cgi-bin/reader/conf.cgi?confid=229",
      SLACcitation   = "%%CITATION = POSCI,GSSI14,023;%%"
}

@article{Pattavina:2016kqn,
      author         = "Pattavina, L.",
      title          = "{Scintillating bolometers for the LUCIFER project}",
      collaboration  = "LUCIFER Collaboration",
      journal        = "J.\ Phys.\ Conf.\ Ser.",
      volume         = "718",
      year           = "2016",
      number         = "6",
      pages          = "062048",
      doi            = "10.1088/1742-6596/718/6/062048",
}
      booktitle      = "{Proceedings, 14th International Conference on Topics in
                        Astroparticle and Underground Physics (TAUP 2015): Torino,
                        Italy, September 7-11, 2015}",
      SLACcitation   = "%%CITATION = 00462,718,062048;%%"

@article{Thomas:2013Th,
      author         = "Thomas, K.~J. and Smith, A.~R. and Chan, Y.~D. and Norman, E.~B. and Wang, B.~S. and Hurley, D.~L.",
      title          = "{Low background counting at the LBNL low background facility}",
      journal        = "AIP Conf.\ Proc.",
      volume         = "1549",
      year           = "2013",
      pages          = "20-25",
      doi            = "10.1063/1.4818067",
}

@article{Yanagida:1979as,
      author         = "Yanagida, T.",
      title          = "{Horizontal symmetry and masses of neutrinos}",
      journal        = "Proc.\ Workshop Baryon Number of the Universe and Unified Theories,
      						Tsukuba, Japan, February 1979",
      pages          = "95-99",
      year           = "1979",
      reportNumber   = "KEK-79-18-95",
      SLACcitation   = "%%CITATION = CONFP,C7902131,95;%%",
}
      journal        = "Conf.\ Proc.\ C79-02-13.1",




==> ref_Talks.tex <==
@article{Agostini:2016-Neutrino,
      author         = "Agostini, M.",
      title          = "{First results from GERDA Phase II}",
      year           = "2016",
		note 				= "[To appear in the \href{http://neutrino2016.iopconfs.org/271646}{proceedings of Neutrino 2016}]",
}

@article{Barker:2013qaa,
      author         = "Barker, G.~J. and others",
      title          = "{The Future of Neutrino Mass Measurements: Terrestrial, Astrophysical, and Cosmological 
      						Measurements in the Next Decade. Highlights of the NuMass 2013 Workshop. Milano,
                        Italy, February 4 - 7, 2013}",
      year           = "2013",
      eprint         = "1309.7810",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1309.7810;%%",
}

@article{Blot:2015_SuperNEMO,
      author         = "Blot, S.",
      title          = "{Recent results from the NEMO-3 experiment and the status of SuperNEMO}",
      year           = "2015",
		note 				= "[To appear in the proceedings of the XIV International Conference on Topics in Astroparticle 
								and Underground Physics (\href{http://taup2015.to.infn.it/scientific-program/parallel-sessions/}%
								{TAUP 2015}), Torino, Italy, September 2015]",
}

@article{Elliott:2016_MJD,
      author         = "Elliott, S.",
      title          = "{Initial Results from the MAJORANA DEMONSTRATOR}",
      year           = "2016",
		note 				= "[To appear on \href{http://neutrino2016.iopconfs.org/271646}{J.\ Phys.\ Conf.\ Ser.}]",
}

@article{Ji:2015_PandaX,
      author         = "Ji, X.",
      title          = "{PandaX and 0nuDBD}",
      year           = "2015",
		note 				= "[Presentation at the International Workshop on Baryon and Lepton Number Violation 
								(\href{http://www.physics.umass.edu/blv2015/workshop/program-description/thursday}{BLV 2015}),
								Amherst, MA, USA, April 2015]",
}

@article{Kim:2015_AMoRE,
      author         = "Kim, Y.~H.",
      title          = "{The AMoRE project}",
      year           = "2015",
		note 				= "[To appear in the proceedings of the XIV International Conference on Topics in Astroparticle 
								and Underground Physics (\href{http://taup2015.to.infn.it/scientific-program/parallel-sessions/}%
								{TAUP 2015}), Torino, Italy, September 2015]",
}

@article{Laing:2015_NEXT,
      author         = "Laing, A.",
      title          = "{The NEXT double beta decay experiment}",
      year           = "2015",
		note 				= "[To appear in the proceedings of the XIV International Conference on Topics in Astroparticle 
								and Underground Physics (\href{http://taup2015.to.infn.it/scientific-program/parallel-sessions/}%
								{TAUP 2015}), Torino, Italy, September 2015]",
}

@article{Licciardi:2016_nEXO,
      author         = "Licciardi, C.",
      title          = "{The sensitivity of the nEXO experiment to majorana neutrinos}",
      year           = "2016",
		note 				= "[To appear on \href{http://neutrino2016.iopconfs.org/271646}{J.\ Phys.\ Conf.\ Ser.}]",
}

@article{Ostrovskiy:2015_nEXO,
      author         = "Ostrovskiy, I.",
      title          = "{nEXO: The next generation \ce{^{136}Xe} neutrinoless double beta decay search}",
      year           = "2015",
		note 				= "[To appear in the proceedings of the XIV International Conference on Topics in Astroparticle 
								and Underground Physics (\href{http://taup2015.to.infn.it/scientific-program/parallel-sessions/}%
								{TAUP 2015}), Torino, Italy, September 2015]",
}

@article{Pattavina:2015_LUCIFER,
      author         = "Pattavina, L.",
      title          = "{Scintillating bolometers for the LUCIFER project}",
      year           = "2015",
		note 				= "[To appear in the proceedings of the XIV International Conference on Topics in Astroparticle 
								and Underground Physics (\href{http://taup2015.to.infn.it/scientific-program/parallel-sessions/}%
								{TAUP 2015}), Torino, Italy, September 2015]",
}

@article{Wright:2016_0nbb_future,
      author         = "Wright, A.",
      title          = "{Future neutrinoless double beta decay search experiments}",
      year           = "2016",
		note 				= "[To appear on \href{http://neutrino2016.iopconfs.org/271646}{J.\ Phys.\ Conf.\ Ser.}]",
}

@article{Yang:2016_EXO-200,
      author         = "Yang, L.",
      title          = "{Status and prospects for the EXO-200 and nEXO experiments}",
      year           = "2016",
		note 				= "[To appear on \href{http://neutrino2016.iopconfs.org/271646}{J.\ Phys.\ Conf.\ Ser.}]",
}



==> ref_Theses.tex <==
@article{Delloro_PhD-thesis:2017,
      author         = "Dell'Oro, S.",
      title          = "{Optimization of the CUORE detector during the commissioning phase}",
      journal        = "http://inspirehep.net/record/1615290/",
      year           = "2017",
      url                = "http://inspirehep.net/record/1615290/",
        note                 = "Ph.\,D.\ thesis, INFN - GSSI",
}
https://cuore.lngs.infn.it/en/publications/theses


@article{Fundoni_PhD-thesis:2012,
      author         = "Fundoni, G.",
      title          = "{The relations between Sardinia and the Iberian Peninsula between Late Bronze Age and early Iron Age 
      						through the archaeological evidence (VII - XII centuries B.\,C.) (in Italian)}",
      year           = "2012",
		note 				= "[Ph.\,D.\ thesis, University of C\'ordoba]",
}

@article{Giachero_PhD-thesis:2008,
      author         = "Giachero, A.",
      title          = "{Characterization of cryogenic bolometers and data acquisition system for the CUORE experiment}",
      year           = "2008",
      url				= "http://giachero.mib.infn.it/documents/",
		note 				= "[Ph.\,D.\ thesis, University of Genoa]",
}

@article{Gorla_PhD-thesis:2005,
      author         = "Gorla, P.",
      title          = "{Optimization of the CUORE detector performance}",
      year           = "2005",
		note 				= "[Ph.\,D.\ thesis, University of Milano-Bicocca]",
}

@article{Ouellet_PhD-thesis:2015,
      author         = "Ouellet, J.~L.",
      title          = "{The Search for $0\nu\beta\beta$ Decay in \ce{^{130}Te} with CUORE-0}",
      year           = "2015",
		note 				= "[Ph.\,D.\ thesis, University of California - Berkeley]",
}

@article{Pedretti_PhD-thesis:2004,
      author         = "Pedretti, M.",
      title          = "{The single module for Cuoricino and CUORE detectors: tests, construction and modelling}",
      year           = "2004",
		note 				= "[Ph.\,D.\ thesis, University of Insubria]",
}

@article{Vignati_PhD-thesis:2010,
      author         = "Vignati, M.",
      title          = "{Model of the Response Function of CUORE Bolometers}",
      year           = "2010",
		note 				= "[Ph.\,D.\ thesis, University of Rome - La Sapienza]",
}


==> ref_arXiv.tex <==
@article{CUORECryostat,
      author         = "D'Addabbo, A. and others",
      title          = "{The CUORE cryostat}",
      collaboration  = "CUORE",
      year           = "2018",
      eprint         = "1805.06209",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1805.06209;%%"
}

@article{Abazajian:2012ys,
      author         = "Abazajian, K.~N. and others",
      title          = "{Light Sterile Neutrinos: A White Paper}",
      year           = "2012",
      eprint         = "1204.5379",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-12-881-PPD",
      SLACcitation   = "%%CITATION = ARXIV:1204.5379;%%"
}

@article{Alenkov:2015dic,
      author         = "Alenkov, V. and others",
      title          = "{Technical Design Report for the AMoRE $0\nu\beta\beta$ Decay Search Experiment}",
      collaboration  = "AMoRE Collaboration",
      year           = "2015",
      eprint         = "1512.05957",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1512.05957;%%"
}

@article{Alessandria:2011rc,
      author         = "Alessandria, F. and others",
      title          = "{Sensitivity of CUORE to Neutrinoless Double-Beta Decay}",
      collaboration  = "CUORE Collaboration",
      year           = "2011",
      eprint         = "1109.0494",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = ARXIV:1109.0494;%%"
}

@article{Amendola:2016saw,
      author         = "Amendola, L. and others",
      title          = "{Cosmology and Fundamental Physics with the Euclid Satellite}",
      collaboration  = "Euclid Theory Working Group",
      year           = "2016",
      eprint         = "1606.00180",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1606.00180;%%"
}

@article{Anelli:2015pba,
      author         = "Anelli, M. and others",
      title          = "{A facility to Search for Hidden Particles (SHiP) at the CERN SPS}",
      collaboration  = "SHiP Collaboration",
      year           = "2015",
      eprint         = "1504.04956",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      reportNumber   = "CERN-SPSC-2015-016, SPSC-P-350",
      SLACcitation   = "%%CITATION = ARXIV:1504.04956;%%",
}

@article{Ashenfelter:2015uxt,
      author         = "Ashenfelter, J. and others",
      title          = "{The PROSPECT Physics Program}",
      collaboration  = "PROSPECT Collaboration",
      year           = "2015",
      eprint         = "1512.02202",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1512.02202;%%"
}

@article{Capozzi:2017ipn,
      author         = "Capozzi, F. and Di Valentino, E. and Lisi, E. and Marrone, A. and Melchiorri, A. and Palazzo, A.",
      title          = "{Global constraints on absolute neutrino masses and their ordering}",
      year           = "2017",
      eprint         = "1703.04471",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1703.04471;%%"
}

@article{Deppisch:2015cua,
      author         = "Deppisch, F.~F. and Graf, L. and Kulkarni, S. and Patra, S. and Rodejohann, W. and Sahu, 
      					N. and Sarkar, U.",
      title          = "{Reconciling the 2 TeV Excesses at the LHC in a Linear Seesaw Left-Right Model}",
      year           = "2015",
      eprint         = "1508.05940",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1508.05940;%%"
}

@article{Deppisch:2016scs,
      author         = "Deppisch, F.~F. and Hati, C. and Patra, S. and Pritimita, P. and Sarkar, U.",
      title          = "{Implications of the diphoton excess on Left-Right models and gauge unification}",
      year           = "2016",
      eprint         = "1601.00952",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1601.00952;%%"
}

@article{Doe:2013jfe,
      author         = "Doe, P.~J. and others",
      title          = "{Project 8: Determining neutrino mass from tritium beta decay using a frequency-based method}",
      collaboration  = "Project 8 Collaboration",
      year           = "2013",
      eprint         = "1309.7093",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = ARXIV:1309.7093;%%"
}
      booktitle      = "{Proceedings, Community Summer Study 2013: Snowmass on
                        the Mississippi (CSS2013): Minneapolis, MN, USA, July
                        29-August 6, 2013}",

@article{Gariazzo:2015rra,
      author         = "Gariazzo, S. and Giunti, C. and Laveder, M. and Li, Y.~F. and Zavanin, E.~M.",
      title          = "{Light sterile neutrinos}",
      year           = "2015",
      eprint         = "1507.08204",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1507.08204;%%"
}

@article{Konieczka:2015ela,
      author         = "Konieczka, M. and Baczyk, P. and Satula, W.",
      title          = "{Beta-decay study within multi-reference density functional theory and beyond}",
      year           = "2015",
      eprint         = "1509.04480",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1509.04480;%%"
}

@article{Osipowicz:2001sq,
      author         = "Osipowicz, A. and others",
      title          = "{KATRIN: A Next generation tritium beta decay experiment
                        with sub-eV sensitivity for the electron neutrino mass.
                        Letter of intent}",
      collaboration  = "KATRIN Collaboration",
      year           = "2001",
      eprint         = "hep-ex/0109033",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = HEP-EX/0109033;%%"
}

@article{Rodejohann:2002ng,
      author         = "Rodejohann, W.",
      title          = "{Measuring leptonic CP violation in neutrinoless double beta decay}",
      year           = "2002",
      eprint         = "hep-ph/0203214",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DO-TH-02-01",
      SLACcitation   = "%%CITATION = HEP-PH/0203214;%%",
}

@article{Strumia:2006db,
      author         = "Strumia, A. and Vissani, F.",
      title          = "{Neutrino masses and mixings and \dots}",
      year           = "2006",
      eprint         = "hep-ph/0606054",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFUP-TH-2004-1",
      SLACcitation   = "%%CITATION = HEP-PH/0606054;%%",
}

@article{Wang:2015raa,
      author         = "Wang, G. and others",
      title          = "{CUPID: CUORE (Cryogenic Underground Observatory for Rare 
                        Events) Upgrade with Particle IDentification}",
      collaboration  = "CUPID Collaboration",
      year           = "2015",
      eprint         = "1504.03599",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1504.03599;%%"
}

@article{Wang:2015taa,
      author         = "Wang, G. and others",
      title          = "{R\&D towards CUPID (CUORE Upgrade with Particle IDentification)}",
      collaboration  = "CUPID Collaboration",
      year           = "2015",
      eprint         = "1504.03612",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1504.03612;%%"
}



==> ref_web.tex <==
@misc{Te-price,
		title				="{https://www.metalprices.com}",
		year				="2016",
		url				="{https://www.metalprices.com/metal/tellurium/tellurium-99-99-ex-china}"
}


@misc{PT415-RM,
		author              ="{Cryomech, Inc., ``PT415-RM Supporting Documentation''}",
        title				="{http://www.cryomech.com/specificationsheet/ PT415RM\_ss.pdf}",
        year            ="{2011}",
		url				="{http://www.cryomech.com/specificationsheet/PT415RM\_ss.pdf}",
}

%http://www.cryomech.com/specificationsheet/PT415RM_ss.pdf
%Smith, Jess. "Cherry Pie for Beginners". Pies for Everyone. The Baking Company, 2005. Web. 25 luglio 2007. http://www.piesforeveryone.com
